Fast and Slow Mixing of the Kawasaki Dynamics on Bounded-Degree Graphs

We study the worst-case mixing time of the global Kawasaki dynamics for the fixed-magnetization Ising model on the class of graphs of maximum degree $\Delta$. Proving a conjecture of Carlson, Davies, Kolla, and Perkins, we show that below the tree uniqueness threshold, the Kawasaki dynamics mix rapidly for all magnetizations. Disproving a conjecture of Carlson, Davies, Kolla, and Perkins, we show that the regime of fast mixing does not extend throughout the regime of tractability for this model: there is a range of parameters for which there exist efficient sampling algorithms for the fixed-magnetization Ising model on max-degree $\Delta$ graphs, but the Kawasaki dynamics can take exponential time to mix. Our techniques involve showing spectral independence in the fixed-magnetization Ising model and proving a sharp threshold for the existence of multiple metastable states in the Ising model with external field on random regular graphs.

==> plot-data.tex <==
6.122448979591837e-8	6.2125482376816965e-9
0.0009201537616788803	2.0373300339363664e-7
0.0018402462988679647	2.0802290611986619e-7
0.002760338836057049	2.4640713823043885e-7
0.0036804313732461333	2.467454619648422e-7
0.004600523910435217	2.3164230920260558e-7
0.005520616447624302	2.7835410692256247e-7
0.006440708984813387	2.525361246621855e-7
0.007360801522002471	2.5401467765608214e-7
0.008280894059191555	2.5151007991073557e-7
0.00920098659638064	6.595107550135203e-8
0.010121079133569725	7.264733556382378e-8
0.011041171670758809	7.936225930328457e-8
0.011961264207947893	6.45719354885974e-8
0.012881356745136976	6.96362754278184e-8
0.013801449282326062	7.471476528942774e-8
0.014721541819515146	7.980745634307662e-8
0.01564163435670423	6.368580009837648e-8
0.016561726893893316	4.6106005638582895e-9
0.0174818194310824	4.638649179556195e-9
0.018401911968271484	1.3274587763044267e-7
0.019322004505460566	1.3957937201800451e-7
0.02024209704264965	1.4643205422740988e-7
0.021162189579838737	2.629286739487997e-8
0.02208228211702782	2.747482220436895e-8
0.023002374654216902	2.8660108413828628e-8
0.023922467191405988	2.984873831435308e-8
0.024842559728595073	3.104072426642529e-8
0.025762652265784156	5.7118572378193963e-8
0.02668274480297324	5.9242582234914e-8
0.027602837340162327	5.753681656216113e-8
0.02852292987735141	6.932411188482324e-8
0.029443022414540495	7.16623503884006e-8
0.03036311495172958	7.40072235033617e-8
0.03128320748891866	7.63587560513892e-8
0.032203300026107745	7.871697299306841e-8
0.033123392563296834	8.108189942624379e-8
0.03404348510048592	8.345356059341582e-8
0.034963577637675006	1.3707004391256653e-9
0.03588367017486409	1.3858734380599038e-9
0.03680376271205317	2.6710009363994918e-8
0.03772385524924225	2.7417166451511776e-8
0.038643947786431335	2.8126347542678503e-8
0.03956404032362042	7.039348215691469e-10
0.040484132860809506	7.178698697550552e-10
0.041404225397998595	7.318179933006521e-10
0.04232431793518768	7.457791813441946e-10
0.04324441047237676	4.0326901517192164e-9
0.04416450300956584	4.068372035649645e-8
0.045084595546754924	4.1591596929254445e-8
0.046004688083944006	8.017543642345131e-10
0.04692478062113309	8.157807255942464e-10
0.04784487315832218	8.298201013192365e-10
0.04876496569551127	8.438724622145935e-10
0.04968505823270035	8.57937785584519e-10
0.051525243307078514	8.861074126381799e-10
0.052445335844267596	9.002116355714736e-10
0.053365428381456685	9.143289214379539e-10
0.054285520918645774	1.0155374443403103e-7
0.05520561345583486	1.0342670178923268e-7
0.05612570599302394	9.872354726278477e-8
0.05704579853021302	1.0048969855387695e-7
0.0579658910674021	1.0317056558243799e-7
0.05888598360459119	1.016827634520437e-7
0.05988346934915033	1.0357082786241187e-7
0.06088095509370947	1.0216911122122466e-7
0.06187844083826861	1.040098173131288e-7
0.06287592658282774	1.0305357116306549e-7
0.06387341232738689	1.0321858324334442e-7
0.06487089807194601	5.693476369500597e-10
0.06586838381650514	5.837087955634022e-10
0.06686586956106429	5.980851775321085e-10
0.06786335530562343	6.124769075836793e-10
0.06886084105018256	2.663169561381842e-10
0.0698583267947417	4.4198316042955616e-10
0.07085581253930084	6.763566107644465e-10
0.07185329828385997	6.541858831264161e-10
0.07285078402841912	6.643481372664573e-10
0.07384826977297826	6.745431791257972e-10
0.07484575551753739	3.957986844521644e-9
0.07584324126209652	4.0172958385801625e-9
0.07684072700665566	4.076796883296466e-9
0.0778382127512148	4.727837626024763e-9
0.07883569849577393	4.7962867971244414e-9
0.07983318424033306	4.864958425693233e-9
0.0808306699848922	4.933853508618894e-9
0.08182815572945135	5.002973047993353e-9
0.08282564147401048	3.9932784280475754e-10
0.0838231272185696	3.632604328507847e-10
0.08482061296312875	3.759108011204597e-10
0.08581809870768789	3.8856965190491545e-10
0.08681558445224702	4.0123700287094236e-10
0.08781307019680616	2.1426925007601507e-7
0.0888105559413653	2.170624586685419e-7
0.08980804168592443	2.1986482641870384e-7
0.09080552743048358	2.2267639504490916e-7
0.09180301317504272	2.732277240443546e-8
0.09280049891960185	2.766584769441028e-8
0.09379798466416099	3.8261482777963944e-8
0.09479547040872013	3.3501743335658694e-8
0.09579295615327926	2.70348322721492e-11
0.0967904418978384	1.2050194999821406e-10
0.09778792764239755	1.219488494560994e-10
0.09878541338695668	1.2340056609651723e-10
0.0997828991315158	1.2485712304911392e-10
0.10078038487607495	1.2631854243161378e-10
0.10177787062063409	1.2778484665086168e-10
0.10277535636519322	3.892546726032012e-8
0.10377284210975235	3.9370000856401854e-8
0.10477032785431149	4.065378697040731e-8
0.10576781359887064	6.208003652372796e-8
0.10676529934342976	5.038086795799815e-8
0.1077627850879889	1.0931306479074217e-7
0.10876027083254804	3.8289531247887964e-8
0.10975775657710718	3.870687002018737e-8
0.11075524232166631	3.7035369603264736e-9
0.11175272806622544	1.2913356871082266e-11
0.11275021381078458	1.305102907978491e-11
0.11374769955534372	1.3189169230145199e-11
0.11474518529990285	1.3327779418287333e-11
0.11574267104446198	1.3466861812615656e-11
0.11674015678902112	1.3606419087495528e-11
0.11773764253358027	8.963518784270892e-10
0.1187351282781394	8.107640236260094e-10
0.11973261402269854	8.189957363911408e-10
0.12073009976725768	8.272557020192842e-10
0.12172758551181681	8.35544056397112e-10
0.12272507125637595	8.43860939169864e-10
0.12365645531034597	8.516525557694665e-10
0.12458783936431597	6.364369257300106e-10
0.12551922341828597	6.422438894361966e-10
0.12645060747225598	6.480696182244634e-10
0.12738199152622598	7.663689043900985e-10
0.12831337558019598	1.315297522228494e-10
0.12924475963416598	1.327024650466894e-10
0.130176143688136	2.854920440678588e-10
0.131107527742106	2.8800909949768433e-10
0.13203891179607602	2.9053435756746604e-10
0.13297029585004602	4.070266945440907e-7
0.13390167990401602	3.5596719637380445e-8
0.13483306395798603	7.204043044976386e-10
0.13576444801195603	7.26585948236195e-10
0.13669583206592603	7.605228281628203e-11
0.13762721611989603	7.669806456611639e-11
0.13855860017386604	7.73459713522088e-11
0.13948998422783604	5.078047776834367e-11
0.14042136828180604	5.120509398437445e-11
0.14135275233577604	5.163111388081787e-11
0.14228413638974605	5.205854367376639e-11
0.14321552044371605	5.24873904466742e-11
0.14414690449768608	5.291766056019405e-11
0.14507828855165608	8.24918027116095e-10
0.14600967260562608	3.040648753616093e-9
0.14694105665959611	3.0652182615026335e-9
0.14787244071356612	2.086605625690087e-8
0.14880382476753612	2.1033085134586446e-8
0.14973520882150612	3.7925069710833165e-10
0.15066659287547612	2.8156122977111377e-11
0.15159797692944613	2.8378428368798964e-11
0.15252936098341613	3.095903206828028e-11
0.15346074503738613	2.228348994041951e-11
0.15439212909135613	2.2457086682146445e-11
0.15532351314532614	2.263127004952884e-11
0.15625489719929614	2.2806043078332783e-11
0.15718628125326614	3.895384130999287e-11
0.15811766530723614	3.925209766594828e-11
0.15904904936120617	3.955136782321511e-11
0.15998043341517618	3.9851657275084364e-11
0.16091181746914618	4.0152970792045606e-11
0.1618432015231162	4.0455313722829546e-11
0.1627745855770862	3.2581078893839654e-11
0.16370596963105621	3.282441918099621e-11
0.16463735368502622	1.2748867167395686e-10
0.16556873773899622	1.2843327197471313e-10
0.16650012179296622	9.777020078954868e-11
0.16743150584693622	3.1838316994399946e-10
0.16836288990090623	3.207146463910885e-10
0.16929427395487623	3.2305418785673795e-10
0.17022565800884623	3.254018348178289e-10
0.17115704206281623	1.4207742968230797e-10
0.17208842611678624	1.4310217666517927e-10
0.17301981017075624	1.4413049125143923e-10
0.17395119422472624	1.451623919448049e-10
0.17488257827869624	5.455045978009868e-11
0.17581396233266625	5.4938186812292233e-11
0.17674534638663625	5.532727271120863e-11
0.17767673044060625	3.66069822024806e-11
0.17860811449457625	3.6864413720712655e-11
0.17953949854854626	8.693274413408095e-11
0.18047088260251626	8.753984516440827e-11
0.1814022666564863	8.814909045751218e-11
0.1823336507104563	1.4261500553997921e-9
0.1832467647064902	1.435814785353632e-9
0.18415987870252415	1.4455131573780828e-9
0.1850729926985581	1.480252105207543e-9
0.18598610669459203	1.4901861018305298e-9
0.18689922069062598	1.4863053302583786e-9
0.1878123346866599	1.4800011083569245e-9
0.1887254486826938	1.1220321370515132e-9
0.18963856267872775	1.1294676484594848e-9
0.1905516766747617	9.778566926095984e-10
0.19146479067079564	1.5635418365115652e-9
0.19237790466682958	1.5738083643015062e-9
0.1932910186628635	8.470874248628971e-8
0.1942041326588974	8.526152262148671e-8
0.19511724665493135	8.58162644768979e-8
0.19694347464699924	8.693167467627236e-8
0.19785658864303318	8.749236387618587e-8
0.19876970263906713	8.805505650782998e-8
0.19968281663510107	8.861976319348025e-8
0.20059593063113498	3.7743944823308656e-7
0.2015090446271689	3.7983886885262386e-7
0.20242215862320284	3.8224682600764617e-7
0.20333527261923678	2.8849752361086935e-7
0.20424838661527073	1.4754797006110344e-7
0.20516150061130467	1.4847839516604847e-7
0.2060746146073386	1.494121875005977e-7
0.20698772860337256	1.503493652011163e-7
0.20790084259940647	1.5128994654011796e-7
0.2088139565954404	1.5223394992845395e-7
0.20972707059147433	1.3403371967642665e-7
0.21064018458750827	1.3486576004378516e-7
0.21155329858354222	1.500134904666714e-7
0.21246641257957616	1.7708619890666656e-8
0.2133795265756101	1.7817785238870086e-8
0.21429264057164404	1.7927352798511845e-8
0.21520575456767796	1.5782659187113072e-8
0.21611886856371187	1.587924050097283e-8
0.21703198255974582	1.597617960380723e-8
0.21794509655577976	1.6073478479230623e-8
0.2188582105518137	1.3553936338446073e-9
0.21977132454784765	1.3442797748795345e-9
0.2206844385438816	1.1454125593119755e-9
0.22159755253991553	1.1891002194260724e-9
0.22251066653594945	1.233025424243071e-9
0.22342378053198336	1.2771902697386498e-9
0.2243368945280173	2.7981451759228242e-9
0.22525000852405125	1.3662450481290188e-9
0.2261631225200852	1.4111373864086453e-9
0.22707623651611913	1.45627640258318e-9
0.22798935051215308	1.5016625709803575e-9
0.22981557850422094	1.5931835154087748e-9
0.23072869250025485	1.639321922063462e-9
0.2316418064962888	1.6857141454742302e-9
0.23346803448835668	1.7792671652780484e-9
0.23438114848439062	1.8264320859845843e-9
0.23529426248042454	1.873857467158832e-9
0.23620737647645845	2.202840858030161e-8
0.2371204904724924	2.2156623373610937e-8
0.23803360446852634	2.0177150204693246e-9
0.23894671846456028	2.0662005360185093e-9
0.23985983246059422	1.3860628693833592e-8
0.24077294645662814	1.394068890613674e-8
0.2417634536600321	1.4027887824474511e-8
0.2427539608634361	1.4115456385231277e-8
0.24374446806684008	1.420339695135723e-8
0.24473497527024407	1.4291711908412909e-8
0.24572548247364806	1.5614849388850776e-8
0.24671598967705205	1.4729593512145671e-8
0.24770649688045604	1.4820654251608177e-8
0.24869700408386003	1.491210603854356e-8
0.24968751128726402	1.5003951407549956e-8
0.250678018490668	1.5096192918990573e-8
0.251668525694072	1.716985399789577e-8
0.252659032897476	1.727503032505229e-8
0.25364954010088	1.738066329541278e-8
0.25464004730428397	1.748675590994921e-8
0.25662106171109195	1.7700332200761535e-8
0.2576115689144959	1.7807822013534497e-8
0.25860207611789987	1.791578374396319e-8
0.25959258332130386	1.8024220528058538e-8
0.26058309052470785	1.8133135536805407e-8
0.26157359772811184	1.8242531962561838e-8
0.26256410493151583	1.3764309776316487e-8
0.2635546121349198	5.1607546585899594e-8
0.2645451193383238	5.191739868047842e-8
0.2655356265417278	5.222863258576816e-8
0.2665261337451318	5.2541257652802456e-8
0.2675166409485358	3.304351902671561e-9
0.26850714815193977	3.361903337828773e-9
0.26949765535534376	3.4197655624212595e-9
0.27048816255874775	1.4133974949136713e-8
0.27147866976215174	3.788505607028406e-9
0.2724691769655557	3.810988282471986e-9
0.2734596841689597	3.833573125032926e-9
0.2744501913723637	3.856260842189281e-9
0.2754406985757677	3.879052144888558e-9
0.2764312057791717	3.054473190284722e-9
0.2774217129825757	3.107788201579455e-9
0.27841222018597966	2.8275467337590825e-9
0.27940272738938365	2.8794793062719434e-9
0.28039323459278764	2.9316630775885885e-9
0.28138374179619163	2.9840983858266746e-9
0.2823742489995956	3.7446823030768607e-7
0.2833647562029996	3.947393568356794e-7
0.2843552634064036	3.970324620057301e-7
0.2853457706098076	3.7437762234787796e-7
0.2863362778132116	3.765472842254098e-7
0.28732678501661557	3.787269889730931e-7
0.28831729222001956	3.8091680747972363e-7
0.28930779942342355	3.8874627231974823e-7
0.29029830662682754	3.9364613106560384e-7
0.29128881383023153	3.959146647774888e-7
0.2922793210336355	3.9819382738008926e-7
0.2932698282370395	3.981704097155262e-7
0.2942603354404435	6.3846580916377825e-6
0.2952508426438475	0.00006050135542957877
0.2962413498472515	2.990809733899991e-7
0.29723185705065547	3.0079420304507045e-7
0.29822236425405946	3.0251558267402244e-7
0.29921287145746345	8.964656974085585e-7
0.30020337866086744	8.674029199427254e-7
0.3011938858642714	9.881162148550377e-7
0.3021843930676754	1.941537179875438e-6
0.3031749002710794	1.0141480455765174e-6
0.30416540747448334	1.0409777079318108e-6
0.3050898129872982	5.06283176963088e-7
0.306014218500113	6.326376449938968e-7
0.3069386240129279	5.917760793807661e-7
0.30786302952574274	2.938371468120769e-7
0.3087874350385576	2.953940311240035e-7
0.30971184055137246	5.427184598938696e-7
0.3106362460641873	5.455660369124011e-7
0.3115606515770022	5.546502856109492e-7
0.31248505708981705	5.752150364906826e-7
0.3134094626026319	5.493801037048865e-7
0.3143338681154468	1.2435167658389583e-7
0.31525827362826164	1.2501058966502002e-7
0.3161826791410765	1.2567261095157762e-7
0.31710708465389137	1.2748921200524031e-7
0.3180314901667062	4.586579356369038e-7
0.31895589567952104	8.159934095554054e-6
0.3198803011923359	1.2003666531094503e-7
0.3208047067051507	7.544515161911347e-9
0.3217291122179656	4.488493747716257e-8
0.32265351773078044	4.512193375971685e-8
0.3235779232435953	9.585763728871934e-8
0.32450232875641016	9.636313868272868e-8
0.325426734269225	9.687108737270349e-8
0.3263511397820399	9.738150152446548e-8
0.32727554529485475	7.342079961579915e-8
0.3281999508076696	7.541620330435744e-8
0.3291243563204845	7.581310888302192e-8
0.33004876183329934	9.468114782988076e-8
0.3309731673461142	9.517909395464119e-8
0.33189757285892907	9.567949482800394e-8
0.3328219783717439	9.618236901637878e-8
0.33374638388455874	9.668773527703333e-8
0.3346707893973736	3.2250821176482466e-8
0.3355951949101884	3.242025505471889e-8
0.3365196004230033	3.259053604934025e-8
0.33744400593581814	8.637213935481805e-7
0.338368411448633	4.6084566510598766e-8
0.33929281696144786	4.7009778831395803e-8
0.3402172224742627	4.7953126010410174e-8
0.3411416279870776	4.8914967501323886e-8
0.34206603349989245	4.989567020992264e-8
0.3429904390127073	5.06744284478023e-8
0.3439148445255222	1.1511089393764934e-6
0.34483925003833704	6.371788820751291e-9
0.3457636555511519	7.987602222587579e-9
0.34668806106396677	6.4964643543785605e-9
0.3476124665767816	6.931800118244257e-8
0.34853687208959644	7.067045846304297e-8
0.3494612776024113	7.204867803107769e-8
0.3503856831152261	7.345315625030574e-8
0.351310088628041	1.3816069899502483e-8
0.35223449414085584	1.280722872557808e-8
0.3531588996536707	2.0489564521093857e-7
0.35408330516648556	2.059670692310177e-7
0.3550077106793004	2.0704412368592578e-7
0.3559321161921153	2.0812685405228133e-7
0.35685652170493015	1.9157286578033927e-7
0.357780927217745	4.2221262418475717e-7
0.3587053327305599	4.244027425389538e-7
0.35962973824337474	4.266043414700528e-7
0.3605541437561896	4.2881751353147964e-7
0.36147854926900447	4.3104235228861645e-7
0.3624029547818193	3.997664479491756e-7
0.36332736029463414	3.884336432123998e-8
0.364329159014819	4.468906136425141e-8
0.3653309577350039	4.49433203779687e-8
0.3663327564551888	2.259617975110072e-8
0.3673345551753737	1.5471576398130306e-8
0.36833635389555863	5.65929313481317e-9
0.36933815261574354	1.632609411500873e-8
0.37033995133592845	1.5926932526473768e-8
0.37134175005611336	7.88993510879258e-9
0.37234354877629827	4.657002786804099e-8
0.3733453474964832	8.352630549267468e-9
0.3743471462166681	8.400290767962075e-9
0.375348944936853	9.92429715019341e-9
0.3763507436570379	6.796716560316862e-8
0.3773525423772228	6.835527677750614e-8
0.37835434109740773	8.264176812456729e-7
0.37935613981759264	8.384122987036951e-7
0.38035793853777755	7.974208915220872e-7
0.38135973725796246	8.089971528872543e-7
0.38236153597814737	8.291013834632888e-7
0.3833633346983323	1.3085263122073374e-7
0.3843651334185172	5.2713555353404e-8
0.3853669321387021	5.060545111385605e-8
0.386368730858887	2.7319232867182696e-8
0.3873705295790719	2.7476123524587205e-8
0.38837232829925683	2.6315250904302593e-8
0.38937412701944174	5.782136446344407e-7
0.39037592573962665	5.869875131685687e-7
0.39137772445981156	5.828338145702054e-7
0.39237952317999647	1.244212685167246e-7
0.3933813219001814	2.2758435059343394e-8
0.3943831206203663	2.2889756512426518e-8
0.3953849193405512	2.3021934864416215e-8
0.3963867180607361	2.3154978716840133e-8
0.397388516780921	8.493129317053026e-8
0.39839031550110593	8.542261382639223e-8
0.39939211422129084	8.591718239993766e-8
0.40039391294147575	8.641503192401003e-8
0.40139571166166066	8.691619588510783e-8
0.40239751038184557	8.069198640381707e-9
0.4033993091020305	8.116108287561436e-9
0.4044011078222154	2.608509644607483e-8
0.4054029065424003	2.6237009049958994e-8
0.4064047052625852	2.6389952270617413e-8
0.4074065039827701	3.330186875287755e-8
0.40840830270295503	5.009922881647471e-6
0.40941010142313994	4.942358022306323e-8
0.41041190014332485	4.971281053823801e-8
0.41141369886350976	5.0004038805002644e-8
0.41241549758369467	1.0735717436364796e-8
0.4134172963038796	9.392840207786544e-8
0.4144190950240645	4.870884650883795e-7
0.4154208937442494	4.3759776191032916e-7
0.4164226924644343	4.40131140524615e-7
0.4174244911846192	4.4268189190720153e-7
0.4184262899048041	4.452501994146831e-7
0.41942808862498904	1.416655812665055e-8
0.42042988734517395	1.4250425429749743e-8
0.42143168606535886	1.3773875331400145e-8
0.42243348478554377	1.8387682357166242e-8
0.4234352835057287	1.8496950670176628e-8
0.4244370822259136	1.6354123206731786e-8
0.4254388809460985	1.6451563509092368e-8
0.4264406796662834	2.3181521931404028e-8
0.4274424783864683	2.2591264292404017e-8
0.42842600704871714	2.172200631214932e-8
0.42940953571096596	2.3779466133684587e-8
0.4303930643732148	2.391951274296074e-8
0.43137659303546366	2.4060584432782097e-8
0.43236012169771254	2.5191761167919542e-8
0.43334365035996136	2.5340765088577064e-8
0.4343271790222102	2.5490872480424394e-8
0.435310707684459	2.4370189212860078e-8
0.43629423634670783	1.3323229047244209e-8
0.4372777650089567	1.34025155584405e-8
0.4382612936712056	1.703656844715121e-8
0.4392448223334544	2.6688509597461096e-8
0.44022835099570323	2.5262583564275256e-8
0.44121187965795206	2.772527780978184e-8
0.4421954083202009	3.2319561742750754e-8
0.44317893698244976	2.5436903739559005e-8
0.44416246564469863	2.3813369792494522e-8
0.44514599430694746	2.5353703468609918e-8
0.4461295229691963	1.6910591333353056e-8
0.4471130516314451	2.1434180254947566e-8
0.4480965802936939	2.141885334465905e-8
0.4490801089559428	2.0971110695391102e-8
0.4500636376181917	2.109867734002968e-8
0.4510471662804405	5.300074780676369e-8
0.4520306949426893	9.512133810994242e-8
0.45301422360493815	9.570261327006327e-8
0.45399775226718697	1.179545084827142e-8
0.45498128092943585	1.1979050346848034e-8
0.4559648095916847	1.5547880776997434e-8
0.45694833825393355	1.5839687088014185e-8
0.4579318669161824	2.4907308384942102e-8
0.4589153955784312	1.845245680262183e-8
0.45989892424068	1.8566901200541514e-8
0.46088245290292884	1.868229349250705e-8
0.46186598156517766	1.879864572378106e-8
0.46284951022742654	2.2611849147586275e-8
0.4638330388896754	1.1892287550840366e-7
0.46481656755192424	1.2156108085326053e-7
0.46580009621417306	1.2426164481833943e-7
0.4667836248764219	1.2702617684799215e-7
0.4677671535386707	1.2985633231293773e-7
0.46875068220091953	1.3275381396354525e-7
0.46973421086316836	1.5179630755941517e-7
0.47071773952541723	1.5030441523683546e-7
0.4717012681876661	1.5363292506943143e-7
0.47268479684991493	1.5307509883656142e-7
0.47366832551216376	1.540301539602534e-7
0.4746518541744126	3.0145068677324643e-6
0.4756353828366614	1.2797183630377568e-7
0.4766189114989102	1.308338826021567e-7
0.47760244016115905	2.5436103875961297e-7
0.4785859688234079	2.516346124736105e-7
0.4795694974856568	8.268984198418038e-8
0.4805530261479056	2.3771589524101875e-8
0.48153655481015445	2.305550477092327e-8
0.48252008347240327	5.096041009596493e-8
0.4835036121346521	1.853435868340275e-8
0.484487140796901	1.7146849011611238e-7
0.48547066945914985	1.1475692255321521e-7
0.4864541981213987	9.617981634849187e-8
0.4874377267836475	9.68167262421778e-8
0.4884212554458963	9.745963002591563e-8
0.490388312770394	9.876376646142314e-8
0.4913057397420537	9.93805263868512e-8
0.49222316671371347	1.0000280569116789e-7
0.49314059368537316	1.0063067996561585e-7
0.49405802065703286	1.0195017327281502e-7
0.49497544762869256	1.0259400195024734e-7
0.49589287460035225	1.0324370476326792e-7
0.49681030157201195	6.227569478273154e-8
0.49772772854367164	6.26726297391847e-8
0.49864515551533134	7.065502080103689e-8
0.49956258248699104	7.110792026754926e-8
0.5004800094586508	6.948840580050944e-8
0.5013974364303104	6.99364506386562e-8
0.5023148634019702	1.4864697046227084e-7
0.5032322903736299	2.328684636822338e-8
0.5041497173452896	4.620733900268414e-8
0.5050671443169493	4.642992027356624e-8
0.5059845712886091	2.48590120209545e-7
0.5069019982602687	2.502097537693087e-7
0.5078194252319285	5.53383009915277e-7
0.5087368522035882	4.96515402286094e-8
0.5096542791752479	4.302950231750369e-8
0.5105717061469076	2.2477931208698247e-7
0.5114891331185674	2.2626559198711417e-7
0.512406560090227	2.365216725035328e-7
0.5133239870618866	2.3809697591435924e-7
0.5142414140335464	2.396879986555354e-7
0.5151588410052061	2.4129498040776883e-7
0.5160762679768658	2.4241378501105275e-7
0.5169936949485255	2.435191462885329e-7
0.5179111219201853	1.798623790204751e-7
0.5188285488918449	1.5845417084745268e-7
0.5197459758635047	1.5953989692414858e-7
0.5206634028351644	1.6063693614520187e-7
0.5215808298068241	1.6174546852848794e-7
0.5224982567784838	1.6993071615139924e-7
0.5234156837501436	1.7111189924985887e-7
0.5243331107218032	1.7230566206872177e-7
0.525250537693463	8.611484157572663e-8
0.5261679646651227	8.928878698767437e-8
0.5270853916367824	7.797015342186095e-8
0.528002818608442	9.947671278458674e-8
0.5289202455801018	1.0348674418189983e-7
0.5298376725517615	2.7331669556352577e-7
0.5307550995234211	1.7258070548383024e-7
0.5316725264950808	4.1559354516235935e-7
0.5325899534667405	3.0550445614999365e-7
0.5335073804384003	3.141045157857224e-7
0.5344248074100599	3.229557848922024e-7
0.5353422343817196	5.835764339135655e-8
0.5362596613533793	5.994250629818003e-8
0.5371770883250391	5.38792136671444e-8
0.5380945152966987	5.5353005158771076e-8
0.5390119422683585	5.687263292315799e-8
0.5399293692400182	5.843972532968716e-8
0.5408467962116779	7.611374859631388e-8
0.5417642231833376	3.542973514368387e-7
0.5426816501549974	3.6237326847187483e-7
0.543599077126657	3.7065369609750944e-7
0.5445165040983168	3.3866282436729754e-7
0.5454339310699765	3.4644023378957396e-7
0.5463513580416361	3.5441639915724937e-7
0.5472687850132959	3.6259702776700437e-7
0.5481862119849557	3.7098801068425873e-7
0.5491036389566153	4.509811965401893e-7
0.550098459135645	4.6595370024639584e-7
0.5510932793146748	4.6721571661475544e-7
0.5520880994937045	2.792060772952874e-6
0.5530829196727343	0.000012326461202539745
0.554077739851764	0.000042571054033504595
0.5550725600307937	4.874575647001862e-7
0.5560673802098235	4.6999854975310867e-7
0.5570622003888533	4.94665263093241e-7
0.5580570205678832	5.09782186614096e-7
0.5590518407469129	5.033850398348001e-7
0.5600466609259427	5.166160057739838e-7
0.5610414811049724	5.300074963959441e-7
0.5620363012840022	5.326547356902571e-7
0.5630311214630319	1.070507494485044e-6
0.5640259416420617	5.402069633561501e-8
0.5650207618210914	4.3795104408553494e-8
0.5660155820001211	4.948740144526571e-8
0.5670104021791509	3.989833871141066e-8
0.5680052223581806	2.5038739501943637e-7
0.5690000425372104	5.407635842530403e-8
0.5699948627162401	5.5473818709475186e-8
0.5709896828952699	8.93944494785561e-8
0.5719845030742996	9.069787339564807e-8
0.5729793232533295	6.922398396821843e-8
0.5739741434323593	7.42467636259056e-8
0.574968963611389	4.790729565232118e-8
0.5759637837904188	5.740967704708457e-8
0.5769586039694485	5.156276544737051e-7
0.5779534241484783	5.226738754353518e-7
0.578948244327508	5.314342309290212e-7
0.5799430645065378	5.237113616539026e-7
0.5809378846855675	5.71235007229893e-7
0.5819327048645972	9.172214830220511e-7
0.582927525043627	5.835611441960833e-7
0.5839223452226567	5.618159866136605e-7
0.5849171654016865	5.899637541239386e-7
0.5859119855807162	5.984043201725705e-7
0.586906805759746	1.2351120740742795e-6
0.5879016259387757	6.031108568750262e-7
0.5888964461178056	5.207670800343137e-7
0.5898912662968354	1.888269563901955e-7
0.5908860864758652	2.0117055105780355e-7
0.5918809066548949	3.256414209730205e-7
0.5928757268339246	3.3801407238380894e-7
0.5938705470129544	2.060725102930881e-7
0.5948653671919841	2.1964897640702072e-7
0.5958601873710139	2.3754623441008492e-7
0.5968550075500436	1.1837745683864503e-7
0.5978498277290734	1.196917636982583e-7
0.5988446479081031	6.992588152307218e-7
0.5998394680871328	6.659728563697274e-7
0.6008342882661627	2.4406491271999887e-7
0.6018291084451926	2.583357142438395e-7
0.6028239286242223	2.6791968925830705e-7
0.603818748803252	2.7858258206412446e-7
0.6048135689822818	2.8081326656640254e-7
0.6058083891613115	2.7689126156780717e-7
0.6068032093403413	2.8999945738907867e-7
0.607798029519371	2.9315644591036574e-7
0.6087928496984008	3.0029753455432193e-7
0.6097876698774305	3.5362309320821855e-7
0.6107824900564602	5.137953984203553e-7
0.61177731023549	7.991918942395491e-7
0.6127721304145198	5.306410325828534e-7
0.6137008489029605	6.599654623801073e-7
0.6146295673914011	1.0131604679258946e-6
0.6155582858798417	5.382680696696342e-7
0.6164870043682824	3.3924024749094115e-7
0.617415722856723	3.475931080503054e-7
0.6183444413451636	3.54471610198064e-7
0.6192731598336043	3.7948838879419497e-7
0.6202018783220449	3.066645866756451e-7
0.6211305968104854	5.83104636428163e-8
0.6220593152989261	5.879749227477392e-8
0.6229880337873668	5.621711036666553e-8
0.6239167522758073	6.476283739914258e-8
0.6248454707642479	5.594563947497754e-8
0.6257741892526886	6.442638527883896e-8
0.6267029077411292	7.417818861237095e-8
0.6276316262295698	8.381959016747133e-8
0.6285603447180104	8.377460190813014e-8
0.629489063206451	9.036883613080292e-8
0.6304177816948917	9.382462059755701e-8
0.6313465001833323	3.506444826685343e-8
0.6322752186717729	3.471917074293197e-8
0.6332039371602136	3.932071123249665e-8
0.6341326556486542	3.899817936186833e-8
0.6350613741370948	3.8711090876873366e-8
0.6359900926255355	4.3953333815012984e-8
0.6369188111139761	4.370539081785965e-8
0.6378475296024168	1.8795835945198104e-7
0.6387762480908574	1.8316023463916234e-7
0.639704966579298	1.5204939335394117e-7
0.6406336850677387	1.6124490907372869e-7
0.6415624035561793	3.109964128276729e-7
0.6424911220446199	2.538339836164639e-7
0.6434198405330604	1.8065802202350088e-7
0.6443485590215011	2.5501121531275995e-7
0.6452772775099418	3.633285903982881e-7
0.6462059959983824	8.011436587330341e-6
0.647134714486823	4.278572154230291e-7
0.6480634329752637	4.4887129607056617e-7
0.6489921514637043	4.297306254806793e-7
0.6499208699521449	4.922874130744521e-7
0.6508495884405856	2.1007615148789786e-6
0.6517783069290262	7.394744704075818e-7
0.6527070254174668	1.8491640336542292e-8
0.6536357439059075	2.07257727500791e-8
0.6545644623943481	2.5636277400212643e-8
0.6554931808827887	2.5791834095119974e-8
0.6564218993712294	3.1733094641442904e-8
0.65735061785967	2.750773052865132e-8
0.6582793363481105	3.63534226219984e-8
0.6592080548365512	3.5145285865579484e-8
0.6601367733249919	4.0673352891144156e-8
0.6610654918134324	4.330417436706086e-8
0.6619942103018731	4.560714430210305e-8
0.6629229287903138	4.9690584824189797e-8
0.6638516472787543	4.8635850900762654e-8
0.664780365767195	6.54333629658699e-8
0.6657090842556357	5.015206395025182e-8
0.6666378027440762	5.234138158941952e-8
0.6675665212325169	5.778529288057688e-8
0.6684952397209576	6.537966216682401e-8
0.6694239582093982	7.944411959348575e-8
0.6703526766978388	8.946475290568217e-8
0.6712813951862795	9.269840229311513e-8
0.6722101136747201	1.226351635969902e-7
0.6731205621052246	1.424242851212669e-7
0.6740310105357292	0.000011264082128915672
0.6749414589662337	1.9536709853983487e-7
0.6758519073967383	0.000023472863172028362
0.6767623558272429	3.0827425461987763e-7
0.6776728042577473	3.5964574869402455e-7
0.6785832526882519	9.760446683430528e-9
0.6794937011187565	1.597294272171426e-8
0.6804041495492611	2.063729715989942e-8
0.6813145979797657	1.6216962795610797e-7
0.6822250464102702	2.2958895886011618e-7
0.6831354948407747	7.124371925631812e-9
0.6840459432712793	1.3648119124277068e-8
0.6849563917017838	2.125913546156992e-8
0.6858668401322884	3.1703397458196895e-8
0.686777288562793	6.662282950859848e-9
0.6876877369932975	7.682794346492223e-9
0.6885981854238021	1.53910853783824e-8
0.6895086338543066	5.041644237039479e-6
0.6904190822848112	1.2921872630862127e-7
0.6913295307153158	1.5895643312968252e-8
0.6922399791458203	5.671579255099473e-9
0.6931504275763248	0.005096637555161041
0.6940608760068294	0.0853012085473507
0.694971324437334	0.12025409926557884
0.6958817728678386	0.14690461367457186
0.6967922212983431	0.16922404685790213
0.6977026697288476	0.18875693705217497
0.6986131181593522	0.20629807861341268
0.6995235665898567	0.2223209732741511
0.7013444634508659	0.25095574956842137
0.7022549118813705	0.26394050041292383
0.703165360311875	0.2762084057392545
0.7049862571728841	0.29894599249140447
0.7058967056033887	0.30954987353652685
0.7068071540338932	0.31971358827646523
0.7086280508949023	0.3388809051399927
0.7095384993254069	0.3479501194915769
0.7104489477559115	0.35671271507066593
0.7122698446169206	0.3734067568899954
0.7159116383389388	0.40395909148067033
0.7168220867694434	0.4110877568107682
0.717732535199948	0.41803523924830643
0.719553432060957	0.4314238808840385
0.7231952257829752	0.4563956386892606
0.7304788132270118	0.5004438307131418
0.7314666548648865	0.5059100753755476
0.7324544965027611	0.5112693474196021
0.7344301797785102	0.5216822149265626
0.7383815463300087	0.5413799997407597
0.7393693879678833	0.5460871471200002
0.7403572296057579	0.5507128119581777
0.7423329128815072	0.559729494903298
0.7462842794330056	0.5768865893454841
0.7472721210708801	0.5810051253065389
0.7482599627087547	0.5850591452454114
0.750235645984504	0.5929799271246889
0.7541870125360024	0.6081172408052993
0.7620897456389993	0.6358761561050064
0.763077587276874	0.6391330018270205
0.7640654289147486	0.6423459997062808
0.7660411121904978	0.6486438483207793
0.7699924787419963	0.6607520907838612
0.7778952118449931	0.6831921720412075
0.7788830534828677	0.6858442103385056
0.7798708951207423	0.6884642770186277
0.7818465783964915	0.6936109392408062
0.7857979449479899	0.7035457909375338
0.7937006780509869	0.7220922383334811
0.7946224179982724	0.7241486190782783
0.7955441579455578	0.7261838745633796
0.7973876378401288	0.7301922630152876
0.8010745976292708	0.7379689568266585
0.8084485172075546	0.7526242799370684
0.8093702571548401	0.7543769907315379
0.8102919971021256	0.7561128749938331
0.8121354769966965	0.7595352388559772
0.8158224367858384	0.7661881125878127
0.8231963563641223	0.778771904440937
0.8241180963114078	0.7802808910472125
0.8250398362586933	0.7817762514570564
0.8268833161532642	0.7847267688211744
0.8305702759424061	0.7904715574936881
0.8379441955206899	0.8013704492234811
0.8526920346772575	0.821048892194813
0.853691167831913	0.8222892304528858
0.8546903009865685	0.823518566736854
0.8566885672958796	0.8259447493803298
0.8606850999145017	0.8306706553165834
0.868678165151746	0.839643063076207
0.8696772983064016	0.8407218428996077
0.8706764314610571	0.8417914702962935
0.8726746977703681	0.8439036720143078
0.8766712303889903	0.8480226153445001
0.8846642956262345	0.8558595357160984
0.88566342878089	0.856803202899876
0.8866625619355455	0.8577392408039121
0.8886608282448566	0.8595885629239857
0.8926573608634787	0.8631983763069908
0.900650426100723	0.8700793694957815
0.9166365565752115	0.8826078862384408
0.9176174196719309	0.8833273187235277
0.9185982827686504	0.8840413815638338
0.9205600089620893	0.8854535955318684
0.9244834613489672	0.8882157752794695
0.9323303661227229	0.8935015107186937
0.9480241756702342	0.9031961019204342
0.9490050387669537	0.9037659938980436
0.9499859018636732	0.904331872955881
0.951947628057112	0.9054517289026356
0.9558710804439898	0.9076447779986898
0.9637179852177455	0.9118515242533826
0.979411794765257	0.9196018612189213
0.9803265561713873	0.9200281828809457
0.9812413175775176	0.920451838387122
0.9830708403897783	0.9212912991997035
0.9867298860142997	0.9229389272253407
0.9940479772633423	0.9261141777161344
1.0086841597614276	0.9320162612671401
1.0095989211675578	0.9323664765194485
1.0105136825736882	0.9327145716848184
1.0123432053859487	0.9334045535073311
1.01600225101047	0.9347599645338139
1.0233203422595127	0.9373757836887175
1.0379565247575981	0.9422514814271905
1.0389486793710985	0.9425658061213209
1.0399408339845988	0.9428781570303982
1.0419251432115997	0.9434970007881972
1.0458937616656012	0.9447116823470331
1.0538309985736043	0.9470521139481639
1.0697054723896104	0.9514005725061653
1.0706976270031108	0.9516585007548359
1.071689781616611	0.9519149252994096
1.073674090843612	0.95242296857766
1.0776427092976135	0.9534209269499879
1.0855799462056166	0.9553462584741687
1.1014544200216227	0.9589321850056323
1.102380472944534	0.9591310817493325
1.1033065258674453	0.9593289833336113
1.1051586317132678	0.9597213035832362
1.1088628434049128	0.9604933583128399
1.1162712667882029	0.9619879425526621
1.1310881135547828	0.9647902150623174
1.1320141664776942	0.9649575027845322
1.1329402194006053	0.9651239004294744
1.1347923252464276	0.9654540655488347
1.1384965369380726	0.9661038966873906
1.1459049603213627	0.9673629963406174
1.1607218070879428	0.9697276439246071
1.161725253218224	0.9698807457686119
1.1627286993485053	0.9700329898339165
1.164735591609068	0.9703349180556218
1.1687493761301933	0.9709286856138432
1.1767769451724437	0.9720770526351713
1.1928320832569446	0.9742261013537563
1.1938355293872258	0.9743541952467596
1.194838975517507	0.9744816074368036
1.1968458677780698	0.974734411530956
1.200859652299195	0.975231553230639
1.2088872213414454	0.976193931742953
1.2249423594259463	0.9779977353913138
1.2259275354982915	0.9781034082941958
1.2269127115706366	0.9782085463701746
1.2288830637153272	0.9784171704223521
1.232823768004708	0.9788278559607589
1.24070517658347	0.9796238240703663
1.2564679937409937	0.9811194446652352
1.2574531698133389	0.9812088501846287
1.2584383458856843	0.9812978041602105
1.2604086980303748	0.9814743389089234
1.2643494023197557	0.9818220421343405
1.2722308108985176	0.9824961837610412
1.2879936280560413	0.983764534246623
1.2889127024377975	0.9838353267215928
1.2898317768195535	0.9839058065570607
1.291669925583066	0.9840457597816813
1.2953462231100903	0.9843217366548751
1.302698818164139	0.9848583122081123
1.3174040082722367	0.9858728800973992
1.318323082653993	0.9859338068067584
1.3192421570357489	0.9859944503325708
1.3210803057992613	0.9861148935116829
1.3247566033262856	0.9863524457619368
1.3321091983803344	0.9868145190714029
1.346814388488432	0.9876889697131006
1.3478108560775581	0.9877459277209825
1.3488073236666844	0.9878026029810145
1.3508002588449366	0.9879151114119822
1.3547861292014414	0.9881368035695589
1.3627578699144505	0.9885672141820164
1.3787013513404691	0.9893787003212803
1.3796978189295952	0.9894273302628259
1.3806942865187213	0.9894757232470787
1.3826872216969737	0.9895718054050406
1.3866730920534782	0.9897611520041214
1.3946448327664875	0.9901289407602228
1.410588314192506	0.9908229448861393
1.411518680091043	0.9908618054209071
1.41244904598958	0.9909004899490969
1.414309777786654	0.9909773384295456
1.418031241380802	0.9911289728479193
1.4254741685690984	0.9914241774456538
1.4403600229456908	0.991983750401288
1.4412903888442279	0.9920174129381901
1.4422207547427648	0.9920509257426022
1.4440814865398388	0.9921175049038012
1.4478029501339869	0.9922488973730879
1.4552458773222832	0.9925047753150327
1.4701317316988756	0.9929901086779273
1.4710438275394764	0.9930187425739643
1.4719559233800774	0.9930472598501947
1.4737801150612793	0.9931039205449714
1.4774284984236832	0.9932157720447604
1.4847252651484908	0.993433788092137
1.499318798598106	0.9938479556568902
1.5002308944387068	0.9938729101293373
1.5011429902793079	0.9938977581963588
1.5029671819605097	0.9939471366721269
1.5066155653229136	0.9940446364948577
1.5139123320477212	0.9942347136548213
1.5285058654973367	0.99459599527548
1.5294953545453076	0.994619614540411
1.5304848435932787	0.9946431254022325
1.5324638216892206	0.9946898244997407
1.5364217778811047	0.9947819461439625
1.5443376902648729	0.994961198827883
1.5601695150324089	0.9953006170741943
1.56115900408038	0.9953210198630532
1.562148493128351	0.9953413302536256
1.564127471224293	0.9953816738061263
1.5680854274161768	0.9954612692445641
1.5760013397999448	0.9956161877156224
1.591833164567481	0.9959096830839412
1.5927565519248628	0.995926155053421
1.5936799392822447	0.9959425577983234
1.5955267139970086	0.9959751571911637
1.599220263426536	0.9960395434530818
1.6066073622855912	0.9961651012129776
1.6075307496429732	0.99618050332227
1.6084541370003549	0.9961958467324575
1.6103009117151186	0.9962263196576249
1.6139944611446462	0.9962865255806285
1.6213815600037011	0.9964039424295438
1.622304947361083	0.9964183457095911
1.6232283347184648	0.9964326893726678
1.6250751094332285	0.9964611971198757
1.6287686588627561	0.9965175043745251
1.6296920462201379	0.9965314388733962
1.6306154335775198	0.9965453113220886
1.6324622082922837	0.9965728834135966
1.6333855956496657	0.9965865835614489
1.6343089830070474	0.9966002267787483
1.636155757721811	0.9966273434187679
1.637079145079193	0.996640817337106
1.6380025324365748	0.9966542353161383
1.6389259197939565	3.446585885637615e-26
1.6398493071513385	1.0518145402946823e-30
1.6407726945087204	-2.1036290805893647e-30
1.6416960818661024	3.1554436208840472e-30
1.643542856580866	0.
1.6444662439382478	-2.1036290805893647e-30
1.6453896312956298	4.2072581611787294e-30
1.6472364060103937	4.2072581611787294e-30
1.650929955439921	4.2072581611787294e-30
1.6519307360046729	-4.2072581611787294e-30
1.652931516569425	8.414516322357459e-30
1.6549330776989288	4.2072581611787294e-30
1.6589361999579366	0.
1.666942444475952	2.1036290805893647e-30
1.6829549335119829	-4.411629933616147e-24
1.7149799115840445	0.
1.7159624220908603	-2.5679065925163143e-34
1.7169449325976762	0.
1.718909953611308	2.5679065925163143e-34
1.7228399956385714	0.
1.7307000796930982	-2.1541161785235095e-27
1.731682590199914	0.
1.73266510070673	8.616464714094038e-27
1.7346301217203617	0.
1.7385601637476251	0.
1.7395426742544409	0.
1.7405251847612568	0.
1.7415076952680728	1.7232929428188076e-26
1.7424902057748886	9.277600834638016e-10
1.7434727162817043	9.21002706930819e-10
1.7444552267885203	9.142489092956306e-10
1.7454377372953362	9.074991248152179e-10
1.746420247802152	9.007528689636511e-10
1.7474027583089677	8.940106967695693e-10
1.7483852688157837	1.0041656907928943e-9
1.7493677793225997	9.97280132574661e-10
1.7503502898294154	9.903988867587122e-10
1.7513328003362312	9.835214390979175e-10
1.7523153108430471	9.766480825012358e-10
1.7542803318566789	9.629137540618647e-10
1.7552628423634946	9.560523739991881e-10
1.7562453528703106	9.491954192127375e-10
1.7572278633771266	9.423424757681044e-10
1.7582103738839423	9.928532885012948e-10
1.759192884390758	9.859187988599403e-10
1.760175394897574	9.78988251459786e-10
1.76115790540439	9.720621885539988e-10
1.7621404159112057	9.651406300090448e-10
1.7631229264180215	9.865952187158117e-10
1.7641054369248375	9.796295725910893e-10
1.7650879474316534	9.726683232177827e-10
1.7660704579384692	9.797957209715414e-10
1.767052968445285	9.798344268973363e-10
1.768035478952101	9.798374633896357e-10
1.7690179894589169	9.728262672485094e-10
1.7700004999657326	9.658197898813045e-10
1.7709830104725484	1.3332330316662979e-9
1.7719655209793643	1.3254687808685243e-9
1.7729480314861803	1.317710510018754e-9
1.773930541992996	1.3099584498657194e-9
1.7749130524998118	1.3022126729677575e-9
1.7758955630066278	1.2944729606874098e-9
1.7768780735134437	1.2867396849262153e-9
1.7778605840202595	3.7711297174509875e-9
1.778776992836486	3.760148129681134e-9
1.7796934016527128	3.74917820699779e-9
1.7815262192851664	3.727274774231057e-9
1.7851918545500731	3.683611540186917e-9
1.7861082633663	3.672725829944233e-9
1.7870246721825267	3.661852154728037e-9
1.78885748981498	3.640140800519784e-9
1.792523125079887	3.59686281078792e-9
1.7934395338961138	3.5860736553638983e-9
1.7943559427123406	3.5752964107991307e-9
1.796188760344794	3.553778301795372e-9
1.7971051691610205	3.5430376850228456e-9
1.7980215779772473	3.532308966518041e-9
1.7998543956097008	3.510888121423053e-9
1.8007708044259276	3.5001956834699108e-9
1.8016872132421544	3.4895157934296912e-9
1.8026036220583812	3.4788477617141914e-9
1.8035200308746078	3.4681919830215923e-9
1.8044364396908343	1.2513401694286623e-9
1.8053528485070611	1.2444760584583203e-9
1.806269257323288	1.2376162108065052e-9
1.8071856661395147	1.2307604133492687e-9
1.8081020749557415	1.2239094059209828e-9
1.8090184837719683	1.2170625391859574e-9
1.8108513014044216	1.2033816110797993e-9
1.8117677102206482	1.1965476889522143e-9
1.812684119036875	1.1897180662669217e-9
1.8145169366693286	1.176072122190856e-9
1.8154333454855553	1.1692556883390647e-9
1.8163497543017821	1.1624438325324462e-9
1.817266163118009	1.155636256871353e-9
1.8181825719342355	1.1488330226516272e-9
1.819098980750462	1.1420346979445251e-9
1.8200153895666888	1.1352407180903098e-9
1.8209317983829156	1.1284509491170997e-9
1.8218482071991424	3.555768854615621e-9
1.8227646160153692	3.5454640398310464e-9
1.823681024831596	3.535169175494445e-9
1.8255138424640494	3.5146102809400686e-9
1.8291794777289563	3.4736125560423037e-9
1.83651074825877	3.3921037326365122e-9
1.8375045502823668	3.3811049566038727e-9
1.8384983523059635	3.370117859711786e-9
1.840485956353157	3.348180516822238e-9
1.8444611644475442	3.3044503653282174e-9
1.8524115806363184	3.2175720528227715e-9
1.8683124130138669	3.0461613120229533e-9
1.8693062150374637	3.0355524116401516e-9
1.8703000170610604	3.0249563818984795e-9
1.872287621108254	3.0038007618228083e-9
1.876262829202641	2.961636967454967e-9
1.8842132453914153	2.877903275241231e-9
1.9001140777689638	2.712813421170926e-9
1.9010417781019715	2.703279273194084e-9
1.901969478434979	2.6937566927241998e-9
1.9038248791009944	2.6747432238189346e-9
1.9075356804330248	2.636845393964182e-9
1.914957283097086	2.56156767743488e-9
1.9158849834300937	2.552206567874828e-9
1.9168126837631014	2.542855821095331e-9
1.9186680844291166	2.5241876576455856e-9
1.9223788857611472	2.4869798216255303e-9
1.9298004884252085	2.413081867599921e-9
1.9307281887582162	2.4038928086448047e-9
1.9316558890912239	2.394714821999092e-9
1.933511289757239	2.3763903635196947e-9
1.9372220910892697	2.3398706630775645e-9
1.9381497914222774	2.330766736850219e-9
1.939077491755285	2.3216750330383206e-9
1.9409328924213003	2.303521501707977e-9
1.944643693753331	2.2673440835778665e-9
1.9455713940863386	2.2583261959209607e-9
1.9464990944193463	2.2493199441640967e-9
1.9483544950853615	2.2313373357851674e-9
1.9492821954183692	2.2223624719321932e-9
1.9502098957513767	2.2133978065443804e-9
1.9520652964173921	2.1955009365466377e-9
1.9529929967503998	2.186568503507886e-9
1.9539206970834075	2.177646434299573e-9
1.954848397416415	2.1687352745621032e-9
1.9557760977494227	2.1598343724636965e-9
1.9567037980824304	2.150944296996165e-9
1.957631498415438	2.142065209108617e-9
1.9585591987484456	2.467623896487034e-9
1.9594868990814533	2.4583157819622474e-9
1.960396329356525	2.449201657746989e-9
1.9613057596315966	2.440098437831986e-9
1.9631246201817396	2.421924973659983e-9
1.964034050456811	2.412853924892204e-9
1.9649434807318826	2.403793962547295e-9
1.9658529110069543	2.394744758340375e-9
1.9667623412820259	2.385706494795075e-9
1.9676717715570975	4.020017796599121e-9
1.9685812018321691	4.008178077868762e-9
1.9694906321072407	3.996355402240999e-9
1.9704000623823121	3.984549247298293e-9
1.9713094926573835	3.9727586721725145e-9
1.9722189229324552	3.960985821271101e-9
1.9740377834825984	3.937490015984218e-9
1.97494721375767	3.925766182902122e-9
1.9758566440327416	3.9140602523305165e-9
1.9776755045828847	3.8906960451237246e-9
1.981313225683171	3.844166966414559e-9
1.9885886678837437	3.751897904687484e-9
1.989498098158815	3.740438346973806e-9
1.9904075284338867	3.728994778360169e-9
1.99222638898403	3.7061556808006522e-9
1.9958641100843164	3.6606744596905058e-9
2.003139552284889	3.570486589815635e-9
2.017690436686034	3.3931843028078764e-9
2.0186772601684755	3.3813074270200807e-9
2.019664083650917	3.3694481964738908e-9
2.0216377306158004	3.3457852016683625e-9
2.025585024545567	3.2986820274563056e-9
2.0265718480280084	3.2869517427853243e-9
2.02755867151045	3.2752402563611393e-9
2.0295323184753333	3.2518715438689687e-9
2.0334796124051	3.2053530181804046e-9
2.0344664358875413	3.1937692760848536e-9
2.035453259369983	3.1822031147866713e-9
2.0374269063348662	3.1591261768538388e-9
2.038413729817308	3.1476144032496566e-9
2.0394005532997497	3.136119448436381e-9
2.040387376782191	3.1246443331320153e-9
2.0413742002646327	3.113186787824118e-9
2.042361023747074	3.4305543114186713e-9
2.043347847229516	3.4185355994575485e-9
2.044334670711958	3.4065348983770697e-9
2.0453214941943996	3.394552638054356e-9
2.046308317676841	3.382588955005092e-9
2.0472951411592826	3.3706455358655082e-9
2.049268788124166	3.346808386580216e-9
2.050255611606608	3.334919093320398e-9
2.0512424350890495	3.3230465576523713e-9
2.0532160820539325	3.299358151268172e-9
2.0571633759836994	3.2521985709400006e-9
2.0650579638432323	3.158750388553273e-9
2.080847139562298	2.9752909375664773e-9
2.081767861354151	2.9647329842624278e-9
2.082688583146003	2.954189771897551e-9
2.084530026729708	2.9331507149115325e-9
2.088212913897118	2.89125417339548e-9
2.095578688231938	2.808187747879552e-9
2.1103102369015776	2.644930559431903e-9
2.1397733342408576	2.3296319536306406e-9
2.14077144924008	2.319207757922533e-9
2.1417695642393024	2.3087978920288354e-9
2.1437657942377477	2.28803072653798e-9
2.1477582542346383	2.246692004130537e-9
2.1557431742284185	2.1647966298089054e-9
2.171713014215979	2.0040922031706728e-9
2.1727111292152017	1.9941836225510985e-9
2.1737092442144244	1.9842900226409764e-9
2.175705474212869	1.964549234968903e-9
2.1796979342097593	1.9252565491065897e-9
2.1876828542035396	1.8474145657515324e-9
2.1886809692027622	1.8377538914862518e-9
2.189679084201985	1.8281081460155446e-9
2.1916753142004297	1.8088626011378505e-9
2.19566777419732	1.7705542198561302e-9
2.2036526941911005	1.6946609511731066e-9
2.204584707499734	1.6858650870640353e-9
2.205516720808367	1.6770824297988587e-9
2.207380747425634	1.6595552779054925e-9
2.2083127607342674	1.6508106936164526e-9
2.209244774042901	1.642079826153092e-9
2.211108800660168	1.6246570148881822e-9
2.2120408139688013	1.6159643107444955e-9
2.2129728272774347	1.6072854731426056e-9
2.213904840586068	1.5986177642326234e-9
2.2148368538947016	1.589964254408756e-9
2.215768867203335	1.5813230410844637e-9
2.2167008805119686	1.880274517722104e-9
2.217632893820602	1.8712030000001237e-9
2.2185649071292355	1.8621449869085076e-9
2.219496920437869	1.8531005016678138e-9
2.2204289337465024	1.8440696988680661e-9
2.2222929603637693	1.826049433843764e-9
2.223224973672403	1.8170597238164644e-9
2.2241569869810363	1.8080842927710576e-9
2.2260210135983027	1.7901721576745421e-9
2.226953026906936	1.7812368181575987e-9
2.227885040215569	1.772315237107925e-9
2.2288170535242027	1.7634066732909448e-9
2.229749066832836	1.7545110579166366e-9
2.2306810801414696	1.745630295317774e-9
2.231613093450103	1.7367621100856279e-9
2.2325451067587365	1.7279075637766374e-9
2.23347712006737	2.0251524212162258e-9
2.2344091333760034	2.015986911667099e-9
2.235341146684637	2.0068364345721185e-9
2.237205173301904	1.9885768617738444e-9
2.2409332265364372	1.95222051267903e-9
2.2418652398450707	1.943166473759692e-9
2.2427972531537037	1.934125318390813e-9
2.2446612797709706	1.9160840814450343e-9
2.245593293079604	1.907083809826955e-9
2.2465253063882376	1.898098733505178e-9
2.247457319696871	1.889123748641777e-9
2.2483893330055045	1.880164859046679e-9
2.249321346314138	1.8712185338331917e-9
2.2502533596227714	2.145761467301142e-9
2.251185372931405	2.1363277161115348e-9
2.2521173862400383	2.12690897821729e-9
2.253049399548672	2.1175051309465073e-9
2.2539814128573052	2.1081166953751006e-9
2.2558454394745717	2.0893831665692303e-9
2.256777452783205	2.0800393155161187e-9
2.257709466091838	2.0707073361201378e-9
2.259573492709105	2.0520912706769056e-9
2.2605055060177386	2.0428039791433725e-9
2.261437519326372	2.033532954887344e-9
2.2623695326350055	2.0242753605819013e-9
2.263301545943639	2.01503179347626e-9
2.264215289194336	2.0059841310097064e-9
2.2651290324450337	2.408012511597517e-9
2.2660427756957313	2.3982858089851984e-9
2.2669565189464285	2.388575133903463e-9
2.2678702621971256	2.378879004759441e-9
2.268784005447823	2.3692000494390513e-9
2.270611491949218	2.349886810371903e-9
2.271525235199915	2.340254759150189e-9
2.2724389784506127	2.3306361955397856e-9
2.2742664649520075	2.311446310320218e-9
2.2779214379547965	2.2732480787488867e-9
2.278835181205494	2.2637378056223413e-9
2.2797489244561913	2.2542417574463642e-9
2.2815764109575856	2.2352944027850574e-9
2.2824901542082827	2.225843652905886e-9
2.2834038974589803	2.2164079086116863e-9
2.284317640709678	2.2069859300601554e-9
2.285231383960375	2.1975798991013408e-9
2.286145127211072	2.188188547560103e-9
2.28705887046177	2.372355606553936e-9
2.2879726137124674	2.3625985157225085e-9
2.2888863569631646	2.3528561461635157e-9
2.2898001002138617	2.3431285558436525e-9
2.2907138434645593	2.3334180497132336e-9
2.292541329965954	2.31404431305584e-9
2.293455073216651	2.3043813270205465e-9
2.294368816467349	2.2947338021980343e-9
2.2952825597180464	2.2851023171797594e-9
2.2961963029687436	2.2754880420532595e-9
2.2971100462194407	2.2658866066461655e-9
2.2980237894701383	2.3498224299868767e-9
2.298937532720836	2.3400258598611706e-9
2.299851275971533	2.330246709166617e-9
2.30076501922223	2.3204840135001665e-9
2.301678762472928	2.310737912592256e-9
2.3025925057236254	2.346986589038761e-9
2.3035062489743225	2.3371420226352295e-9
2.3044199922250197	2.327314586188449e-9
2.305333735475717	2.340244231133687e-9
2.306247478726414	2.3416970120613072e-9
2.3071612219771116	2.3402569865772838e-9
2.308074965227809	2.3331465816115853e-9
2.3089887084785063	2.3232386275808e-9
2.3108161949799007	2.303474746073783e-9
2.31447116798269	2.264149531123766e-9
2.321781113988269	2.186312533405227e-9
2.3227722504463366	2.1758413422419572e-9
2.323763386904404	2.1653896520160224e-9
2.3257456598205386	2.144544625727089e-9
2.329710205652808	2.103085892855905e-9
2.3376392973173474	2.0210889289253225e-9
2.3534974806464257	1.8606925471506603e-9
2.3852138473045827	1.5536555644471774e-9
2.444416072423192	1.0256719499052053e-9
2.5085714628134843	5.124591696658345e-10
2.5095556207303966	5.050200461890429e-10
2.510539778647309	4.975951584077651e-10
2.5125080944811335	4.827810419379735e-10
2.5164447261487823	4.533000972347197e-10
2.5243179894840804	3.9492942946753804e-10
2.5400645161546764	2.8049819416227194e-10
2.5410486740715887	2.7344682089340415e-10
2.542032831988501	2.664065065149919e-10
2.5440011478223257	2.5236226627402917e-10
2.5479377794899745	2.2441201226978992e-10
2.5558110428252725	1.6906143678462091e-10
2.556795200742185	1.621926650788066e-10
2.557779358659097	1.553358488765334e-10
2.5597476744929213	1.4165751178567762e-10
2.56368430616057	1.144336835425315e-10
2.571557569495868	6.051742979487386e-11
2.5724756257221912	5.427620033962751e-11
2.573393681948514	4.804551236381678e-11
2.57522979440116	3.5610774658718115e-11
2.5761478506274833	2.940754780340959e-11
2.5770659068538064	2.321356910424978e-11
2.5789020193064527	1.0855060386865222e-11
2.579820075532776	4.689663639808156e-12
2.580738131759099	0.
2.581656187985422	8.616464714094038e-27
2.582574244211745	-8.616464714094038e-27
2.5834923004380683	-2.692645223154387e-28
2.5844103566643915	2.692645223154387e-28
2.5862464691170377	0.
2.587164525343361	-2.692645223154387e-28
2.588082581569684	2.692645223154387e-28
2.58991869402233	0.
2.5935909189276227	0.
2.6009353687382077	2.692645223154387e-28
2.601853424964531	2.692645223154387e-28
2.602771481190854	0.
2.6046075936435003	0.
2.6082798185487928	0.
2.615624268359378	-2.692645223154387e-28
2.630313167980548	0.
2.6313086174142413	0.
2.6323040668479343	2.692645223154387e-28
2.6342949657153207	2.692645223154387e-28
2.638276763450093	2.692645223154387e-28
2.6462403589196386	-2.692645223154387e-28
2.6621675498587294	-5.385290446308774e-28
2.694021931736911	-5.385290446308774e-28
2.7535001872955696	0.
2.8118091591463195	-5.385290446308774e-28
2.875071296268753	0.
2.9341029251934816	0.
2.935132566030701	-1.3463226115771934e-28
2.9361622068679196	0.
2.938221488542358	-1.3463226115771934e-28
2.942340051891235	0.
2.950577178588989	1.3234889800848443e-23
2.967051431984496	8.823259867232295e-24
2.968081072821715	1.3234889800848443e-23
2.9691107136589343	8.823259867232295e-24
2.971169995333373	1.3234889800848443e-23
2.9752885586822493	1.764651973446459e-23
2.9835256853800027	0.
2.984555326217222	0.
2.985584967054441	0.
2.9876442487288797	-1.3463226115771934e-28
2.9917628120777566	0.
2.992792452914976	0.
2.993822093752195	0.
2.9958813754266336	0.
2.996911016263853	1.3463226115771934e-28
2.997940657101072	-1.3463226115771934e-28
2.998970297938291	0.
2.99999993877551	0.

==> second-moment-data1.tex <==
0.02168370738915929	1.625615781056906
0.022288623187021427	1.6261906141113904
0.024948585172512458	1.6285449665879976
0.025281080420698838	1.628824253244408
0.025613575668885218	1.6291003963156931
0.026278566165257974	1.6296434625722924
0.02760854715800349	1.630694114503361
0.03026850914349452	1.632663660679473
0.0306010043916809	1.6328983069774874
0.03093349963986728	1.6331305136206111
0.03159849013624004	1.6335877491333788
0.03292847112898555	1.6344744537257583
0.035588433114476584	1.6361437616772716
0.040908357085458646	1.6391137775708926
0.04121881843678198	1.639273443462786
0.04152927978810532	1.6394317090148172
0.042150202490751985	1.639744099786394
0.043392047896045324	1.64035273124943
0.04587573870663201	1.6415084944809968
0.046186200057955346	1.6416474538483028
0.046496661409278675	1.6417852297699864
0.04711758411192535	1.6420572785572167
0.048359429517218694	1.6425876852972539
0.05084312032780537	1.6435961718961971
0.05115358167912871	1.643717528179725
0.051464043030452045	1.6438378717390285
0.05208496573309871	1.6440755583682265
0.05332681113839205	1.6445391864617918
0.05581050194897873	1.6454214174606379
0.06077788357015209	1.6470200045209764
0.0610822549021634	1.6471112679349604
0.06138662623417471	1.6472017975639752
0.06199536889819733	1.6473806792533336
0.06321285422624258	1.6477298951409636
0.06564782488233308	1.648395386091135
0.0659521962143444	1.6484755885944642
0.0662565675463557	1.6485551451823401
0.06686531021037832	1.6487123405541209
0.06808279553842357	1.6490191967556949
0.07051776619451407	1.6496038225033616
0.07082213752652539	1.649674261902281
0.07112650885853669	1.649744129417693
0.07173525152255932	1.6498821657005562
0.07295273685060456	1.6501515592595264
0.07538770750669506	1.6506645247102822
0.08025764881887605	1.65159382919625
0.08058781788667738	1.651652438974897
0.08091798695447872	1.6517105139667225
0.08157832509008137	1.6518250754962018
0.0828990013612867	1.652047953948478
0.08554035390369732	1.6524695753964949
0.08587052297149865	1.65252008619658
0.08620069203929998	1.652570121624825
0.08686103017490264	1.6526687800331827
0.08818170644610795	1.6528605409897597
0.09082305898851858	1.6532225658336717
0.09115322805631991	1.6532658647216563
0.09148339712412124	1.6533087394667536
0.0921437352597239	1.6533932283624289
0.09346441153092921	1.653557245181259
0.09610576407333984	1.6538660654562576
0.10138846915816112	1.6544115878105048
0.10169660432909941	1.6544406029903849
0.10200473950003769	1.6544693212504467
0.10262100984191426	1.6545258743743416
0.1038535505256674	1.6546354978183329
0.10631863189317368	1.654841208672552
0.10662676706411198	1.654865686994435
0.10693490223505026	1.6548898963297034
0.10755117257692683	1.6549375145884757
0.10878371326067997	1.655029594644075
0.11124879462818625	1.655201480907988
0.11155692979912454	1.6552218458598764
0.11186506497006282	1.6552419667154092
0.11248133531193939	1.6552814819862929
0.11371387599569253	1.6553576471487044
0.11617895736319882	1.6554988308356258
0.11648709253413711	1.6555154605195197
0.11679522770507539	1.655531868380104
0.11741149804695196	1.655564023876827
0.1186440387307051	1.6556257302053101
0.12110912009821138	1.6557390069815967
0.12144305300493968	1.6557533391116834
0.121776985911668	1.6557674343364015
0.12244485172512459	1.6557949200739466
0.12378058335203782	1.6558471141490763
0.12411451625876613	1.6558595925585533
0.12444844916549443	1.6558718458037616
0.12511631497895104	1.6558956824813058
0.12645204660586423	1.6559407158035944
0.12678597951259254	1.6559514321870232
0.12711991241932086	1.6559619345175116
0.12778777823277745	1.6559823023980345
0.12912350985969068	1.6560205281823024
0.12945744276641896	1.6560295693518552
0.12979137567314727	1.6560384069937881
0.13045924148660387	1.6560554767923004
0.1317949731135171	1.656087229661187
0.1321289060202454	1.6560946778832257
0.1324628389269737	1.6561019325569348
0.13313070474043032	1.656115866094978
0.1334646376471586	1.6561225473574674
0.13379857055388691	1.6561290398680735
0.1344664363673435	1.6561414633449068
0.13480036927407182	1.6561473966477822
0.13513430218080014	1.6561531458721908
0.13580216799425673	1.6561640966767108
0.13713789962116996	1.6561838394369888
0.13747183252789824	1.656188331893006
0.13780576543462655	1.6561926492645593
0.13847363124808315	1.6562007631167994
0.13880756415481146	1.6562045617615715
0.13914149706153978	1.6562081896501646
0.13980936287499637	1.65621493741262
0.14014329578172469	1.6562180593967668
0.14047722868845297	1.6562210148454126
0.14081116159518128	1.656223804797321
0.1411450945019096	1.656226430284804
0.14147902740863788	1.6562288923337676
0.1418129603153662	1.6562311919637702
0.1424808261288228	1.6562353080136636
0.14280866901623906	1.6562370946993343
0.14313651190365534	1.656238728689356
0.1434643547910716	1.656240210919338
0.14379219767848792	1.656241542319269
0.14412004056590422	1.6562427238135544
0.1444478834533205	1.6562437563210664
0.14477572634073677	1.6562446407551843
0.14510356922815304	1.6562453780238342
0.14543141211556931	1.6562459690295364
0.1457592550029856	1.6562464146694462
0.14608709789040186	1.656246715835392
0.14641494077781814	1.6562468734139195
0.1467427836652344	1.656246888286331
0.14707062655265069	1.6562467613287273
0.14739846944006696	1.6562464934120464
0.14772631232748326	1.6562460854021015
0.14805415521489956	1.6562455381596217
0.14838199810231584	1.6562448525402942
0.1487098409897321	1.6562440293947953
0.14903768387714839	1.656243069568833
0.14936552676456466	1.6562419739031855
0.14969336965198093	1.656240743233737
0.1500212125393972	1.6562393783915113
0.15034905542681348	1.6562378802027158
0.15067689831422976	1.656236249488772
0.15100474120164603	1.6562344870663512
0.1513325840890623	1.656232593747416
0.1516604269764786	1.6562305703392468
0.1519882698638949	1.6562284176444855
0.15231611275131118	1.6562261364611615
0.15297179852614373	1.6562211917981229
0.15329964141356	1.6562185298917376
0.15362748430097628	1.6562157426435173
0.15428317007580886	1.6562097952191597
0.15461101296322516	1.6562066365808297
0.15493885585064143	1.656203355676345
0.15559454162547398	1.6561964300968839
0.15592238451289026	1.656192786925225
0.15625022740030653	1.656189024494109
0.15690591317513908	1.6561811448138737
0.1582172847248042	1.6561639866728746
0.1585451276122205	1.6561594099465573
0.15887297049963678	1.656154719775117
0.15952865627446933	1.6561450019277753
0.16084002782413442	1.6561242358134654
0.16346277092346467	1.656077535493607
0.16376857991401791	1.656071653781728
0.16407438890457116	1.656065682793234
0.1646860068856776	1.6560534750923905
0.16590924284789055	1.6560280113895058
0.16835571477231645	1.6559730053620803
0.1686615237628697	1.6559657570276294
0.1689673327534229	1.6559584275419243
0.1695789507345294	1.6559435270610308
0.17080218669674235	1.6559127735379064
0.17324865862116823	1.6558475620989375
0.17355446761172147	1.6558390724298426
0.1738602766022747	1.6558305091169154
0.17447189458338117	1.6558131633577253
0.1756951305455941	1.6557776077724453
0.17814160247001998	1.6557031382911376
0.18303454631887175	1.6555415223911596
0.18336615304521503	1.6555299892893969
0.18369775977155828	1.6555183853775366
0.18436097322424477	1.6554949670928727
0.18568740012961776	1.6554473023278604
0.1883402539403638	1.655348767180342
0.19364596156185587	1.6551397006546242
0.20425737680483996	1.654679731549423
0.20456694963432018	1.6546655756433102
0.2048765224638004	1.6546513816696042
0.2054956681227608	1.6546228806970187
0.20673395944068162	1.6545654348235057
0.20921054207652331	1.6544488316975385
0.21416370734820667	1.6542092784358164
0.22407003789157337	1.65370852941087
0.24349293774233727	1.6526683964817872
0.26456689268366235	1.6514994428486804
0.2842306782257526	1.6504132475772284
0.305545518858404	1.6492782883849881
0.32647059825508584	1.6482368650772723
0.34598550825253294	1.6473517766633232
0.3671514733405411	1.6465041178195778
0.3674601576481782	1.646492698993876
0.3677688419558153	1.646481308359472
0.36838621057108945	1.6464586118349223
0.3696209478016378	1.6464135589469866
0.3720904222627345	1.6463248231636054
0.3770293711849278	1.6461529043803564
0.3869072690293145	1.645831830004574
0.3872417510727416	1.6458214998787757
0.38757623311616873	1.6458112057224308
0.3882451972030229	1.6457907254896762
0.38958312537673134	1.6457501985351166
0.39225898172414814	1.6456708880543203
0.3976106944189818	1.6455193135963664
0.3979451764624089	1.6455101549386484
0.39827965850583597	1.6455010335398803
0.39894862259269015	1.6454829026692916
0.4002865507663986	1.6454470896776365
0.40296240711381537	1.645377266892705
0.408314119808649	1.6452448976145475
0.4086425118327641	1.6452370934711635
0.4089709038568792	1.645229326325512
0.4096276879051093	1.6452139031507542
0.4109412560015696	1.6451835021231154
0.41356839219449026	1.6451244880860947
0.4188226645803315	1.645013664118398
0.4191510566044466	1.6450070585406364
0.4194794486285617	1.6450004908815063
0.4201362326767918	1.644987469425414
0.4214498007732521	1.6449618826986647
0.42407693696617277	1.6449125397737678
0.429331209352014	1.6448212206395174
0.42963756747926607	1.6448162007645888
0.42994392560651806	1.644811214575675
0.43055664186102216	1.6448013433292668
0.4317820743700303	1.6447820058706066
0.4342329393880466	1.6447449550814246
0.43453929751529863	1.644740476335652
0.4348456556425506	1.6447360315588484
0.4354583718970547	1.6447272439797325
0.43668380440606286	1.644710077187595
0.43913466942407914	1.6446773807383457
0.4394410275513312	1.6446734474766986
0.4397473856785832	1.6446695484441072
0.4403601019330873	1.6446618531280446
0.4415855344420954	1.644646873921197
0.4440363994601117	1.6446185645664206
0.44434275758736375	1.6446151807823688
0.44464911571461574	1.6446118314651643
0.44526183196911984	1.644605236287752
0.446487264478128	1.6445924601513082
0.44893812949614426	1.6445685678042194
0.44927028535918634	1.6445655003574486
0.44960244122222837	1.644562473681874
0.4502667529483124	1.644556542709342
0.45159537640048064	1.6445451707275152
0.45192753226352267	1.6445424298998923
0.45225968812656475	1.6445397299705429
0.45292399985264886	1.6445344528680366
0.4542526233048171	1.6445243901110391
0.4545847791678591	1.6445219768936485
0.4549169350309012	1.6445196046943276
0.4555812467569853	1.6445149834076527
0.4569098702091535	1.644506233680146
0.45724202607219555	1.6445041490060943
0.45757418193523763	1.6445021054627027
0.45823849366132174	1.6444981418220794
0.4595671171134899	1.6444907086984368
0.459899272976532	1.6444889534434373
0.460231428839574	1.644487239424555
0.4608957405656581	1.6444839351457698
0.4612278964287001	1.6444823449109036
0.4615600522917422	1.6444807959622292
0.4622243640178263	1.644477821972319
0.4625565198808683	1.644476396955239
0.4628886757439104	1.644475013272667
0.4635529874699945	1.644472369958148
0.46488161092216274	1.6444675798552624
0.46521376678520476	1.6444664858386433
0.46554592264824685	1.6444654332479114
0.46621023437433096	1.6444634523877284
0.466542390237373	1.6444625241398183
0.46687454610041507	1.644461637360875
0.4675388578264992	1.6444599882517805
0.4678710136895412	1.6444592259423036
0.4682031695525833	1.6444585051431437
0.46853532541562537	1.6444578258643676
0.4688674812786674	1.6444571881159373
0.4691996371417094	1.6444565919077034
0.46953179300475145	1.6444560372494115
0.4698639488677935	1.6444555241506997
0.47019610473083556	1.6444550526210984
0.4705062266970146	1.6444546499034904
0.47081634866319355	1.6444542834386577
0.4711264706293726	1.6444539532341058
0.4714365925955516	1.644453659297255
0.4717467145617306	1.6444534016354484
0.47205683652790964	1.6444531802559463
0.4723669584940886	1.644452995165927
0.47267708046026763	1.6444528463724895
0.47298720242644665	1.6444527338826498
0.4732973243926256	1.6444526577033458
0.47360744635880464	1.6444526178414314
0.47391756832498366	1.644452614303683
0.4742276902911627	1.6444526470967933
0.4745378122573417	1.6444527162273752
0.4748479342235207	1.644452821701962
0.4751580561896997	1.6444529635270049
0.4754681781558787	1.6444531417088777
0.4757783001220577	1.6444533562538706
0.4760884220882367	1.6444536071681919
0.47639854405441573	1.6444538944579759
0.47670866602059475	1.6444542181292687
0.4770187879867738	1.6444545781880444
0.47732890995295274	1.6444549746401884
0.47763903191913176	1.6444554074915136
0.4779491538853108	1.6444558767477477
0.47825927585148975	1.6444563824145393
0.4785693978176688	1.644456924497459
0.4788795197838478	1.6444575030019957
0.4791896417500268	1.6444581179335611
0.47949976371620584	1.6444587692974812
0.48012000764856383	1.6444601813433097
0.48043012961474285	1.6444609420354788
0.4807402515809218	1.6444617391805256
0.48136049551327986	1.6444634428488938
0.4816706174794589	1.644464349381838
0.4819807394456379	1.6444652923869068
0.4826009833779959	1.6444672878317854
0.4829111053441749	1.6444683402805833
0.4832212273103539	1.6444694292194784
0.48384147124271193	1.6444717165846656
0.48508195910742796	1.6444767293798948
0.485392081073607	1.6444780738653058
0.48570220303978595	1.6444794548729569
0.486322446972144	1.6444823264695534
0.48756293483686003	1.6444885080854679
0.48787305680303905	1.6444901448469165
0.488183178769218	1.64449181815769
0.48880342270157606	1.6444952744392518
0.4900439105662921	1.6445026257223263
0.49034794251315905	1.644504516721406
0.49065197446002606	1.6445064428695666
0.4912600383537601	1.6445104006221059
0.492476166141228	1.6445187380108852
0.4949084217161639	1.644537100732822
0.4952124536630309	1.644539554348202
0.49551648560989786	1.6445420431401783
0.49612454950363183	1.6445471262582594
0.49734067729109976	1.6445577146572778
0.49977293286603564	1.6445805802566433
0.5000769648129026	1.644583596789445
0.5003809967597697	1.6445866485078133
0.5009890606535036	1.644592857500958
0.5022051884409715	1.644605697706799
0.5046374440159074	1.644633066887212
0.5095019551657791	1.6446945584740542
0.5098317848484362	1.6446990536410449
0.5101616145310931	1.644703590173509
0.5108212738964071	1.644712787322592
0.5121405926270352	1.6447316778658496
0.5147792300882912	1.644771443115849
0.5200565050108032	1.6448589023766889
0.5203863346934603	1.6448647192293209
0.5207161643761172	1.6448705772999588
0.5213758237414312	1.6448824170700211
0.5226951424720593	1.6449065909429108
0.5253337799333153	1.644956914474792
0.5306110548558273	1.6450654509416878
0.5309188506416211	1.6450721054093578
0.5312266464274151	1.6450787955529924
0.5318422379990031	1.6450922828369487
0.533073421142179	1.645119685168724
0.5355357874285307	1.645176199037819
0.540460520001234	1.6452960477237646
0.540768315787028	1.6453038395668826
0.541076111572822	1.6453116667972814
0.5416917031444098	1.6453274273784233
0.5429228862875857	1.645359372727007
0.5453852525739373	1.6454249577398348
0.5503099851466406	1.6455628844808003
0.5506435786682247	1.6455725522784137
0.5509771721898086	1.6455822612051956
0.5516443592329765	1.6456018023798091
0.5529787333193125	1.645641377541486
0.5556474814919843	1.6457224952416116
0.5609849778373279	1.6458925675662535
0.5716599705280151	1.6462637731680427
0.571987474030287	1.6462758105994193
0.572314977532559	1.6462878864143387
0.5729699845371029	1.6463121531020715
0.5742799985461907	1.646361146053248
0.5769000265643663	1.6464609649088484
0.5821400826007176	1.646667889974842
0.5926201946734201	1.647110506594615
0.6121702494195903	1.6480356895417547
0.6333713592563216	1.6491777008952981
0.6531622996938181	1.6503633128318778
0.6725634788953451	1.6516250771118264
0.6936157131874332	1.6530880568716728
0.7132577780802865	1.6545205545712813
0.7345508980637009	1.656118053619562
0.7544338486478805	1.6576178284202245
0.7739270379960906	1.6590556603212938
0.7950712824348619	1.6605210985559336
0.7953796273573546	1.6605413789366856
0.7956879722798473	1.6605616216017802
0.7963046621248329	1.66060199261467
0.7975380418148039	1.6606822691077245
0.800004801194746	1.6608408927683556
0.80493831995463	1.6611498672443994
0.8052466648771228	1.6611687892329678
0.8055550097996156	1.6611876634905405
0.8061716996446011	1.661225267465723
0.8074050793345722	1.6612998877424872
0.8098718387145142	1.6614467001937445
0.8148053574743983	1.6617299719055645
0.8151395001326811	1.661748629891145
0.8154736427909639	1.6617672182153054
0.8161419281075294	1.6618041838945716
0.8174784987406605	1.6618772573420646
0.8201516400069226	1.6620198581523407
0.8254979225394471	1.6622899238831175
0.8258320651977298	1.6623060938666299
0.8261662078560126	1.6623221770029906
0.8268344931725782	1.6623540803935015
0.8281710638057094	1.6624168190860118
0.8308442050719715	1.6625378889674094
0.8361904876044959	1.6627612728921606
0.8365185402434666	1.662774120244292
0.8368465928824373	1.6627868642876327
0.8375026981603789	1.6628120398151471
0.838814908716262	1.6628611220017486
0.8414393298280279	1.6629540587444658
0.8417673824669987	1.662965172224858
0.8420954351059695	1.6629761714348075
0.842751540383911	1.662997824168049
0.8440637509397939	1.6630397265339372
0.84668817205156	1.6631177525522687
0.8470162246905307	1.6631269492621445
0.8473442773295015	1.6631360197174192
0.8480003826074429	1.6631537787166253
0.849312593163326	1.6631877467820686
0.8496406458022967	1.6631959111986714
0.8499686984412675	1.6632039429462526
0.850624803719209	1.663219605138154
0.8519370142750919	1.663249300964941
0.8522650669140627	1.6632563807184526
0.8525931195530334	1.6632633210838053
0.853249224830975	1.6632767801959378
0.854561435386858	1.6633019874796051
0.8548894880258288	1.6633079276966658
0.8552175406647995	1.6633137214826417
0.855873645942741	1.663324866139356
0.857185856498624	1.6633453581319806
0.8574918752407317	1.6633497875091396
0.8577978939828395	1.6633540830919633
0.8584099314670548	1.66336226979168
0.8587159502091626	1.6633661593561717
0.8590219689512703	1.6633699120214493
0.8596340064354857	1.663377003500685
0.8599400251775934	1.663380340726521
0.860246043919701	1.6633835378768382
0.8608580814039165	1.6633895087243216
0.8611641001460242	1.6633922807965729
0.861470118888132	1.6633949095434037
0.8620821563723473	1.6633997337590862
0.862388175114455	1.6634019275651075
0.8626941938565627	1.6634039747199703
0.8630002125986704	1.6634058743801186
0.8633062313407781	1.6634076256970771
0.8636122500828858	1.6634092278174073
0.8639182688249936	1.663410679882673
0.8642242875671012	1.6634119810294048
0.8645303063092089	1.6634131303890538
0.8648363250513167	1.6634141270879608
0.8651423437934244	1.663414970247309
0.865448362535532	1.6634156589830926
0.8657543812776398	1.6634161924060675
0.8660604000197475	1.6634165696217182
0.8663664187618552	1.6634167897302121
0.866672437503963	1.6634168518263603
0.8669784562460706	1.6634167549995742
0.8672844749881783	1.6634164983338238
0.8675904937302861	1.663416080907596
0.8678965124723937	1.6634155017938501
0.8682025312145014	1.663414760059975
0.8685085499566092	1.663413854767744
0.8688145686987169	1.663412784973272
0.8691205874408245	1.6634115497269704
0.8694266061829323	1.6634101480734997
0.86973262492504	1.6634085790517266
0.8700386436671477	1.6634068416946761
0.8703446624092555	1.6634049350294846
0.8706506811513631	1.6634028580773543
0.8709566998934708	1.6634006098535024
0.8712627186355786	1.6633981893671166
0.8718747561197939	1.6633928276130454
0.8721807748619016	1.6633898843331385
0.8724867936040093	1.663386764766155
0.8730988310882247	1.663379992677795
0.8734048498303324	1.6633763380939597
0.8737108685724402	1.6633725030980222
0.8743229060566555	1.6633642876739403
0.8746289247987633	1.66335990513143
0.874934943540871	1.66335533794799
0.8755469810250864	1.6633456453562316
0.8767710559935172	1.6633239967769053
0.8771028724714149	1.6633176012886948
0.8774346889493128	1.6633109782783506
0.8780983219051082	1.6632970439168835
0.879425587816699	1.663266380844855
0.8797574042945967	1.6632581242623004
0.8800892207724944	1.6632496283435643
0.8807528537282899	1.6632319123917811
0.8820801196398809	1.6631935406819263
0.8824119361177786	1.6631833261347966
0.8827437525956763	1.6631728597542503
0.8834073855514717	1.6631511650301507
0.8847346514630626	1.6631046818342536
0.8873891832862444	1.6629989631326614
0.8877209997641421	1.6629845190072852
0.8880528162420398	1.6629697957861267
0.8887164491978353	1.6629395047923603
0.8900437151094263	1.6628754929834515
0.890375531587324	1.6628587645692225
0.8907073480652217	1.6628417421708297
0.8913709810210171	1.6628068077069718
0.892698246932608	1.6627333252780354
0.8930300634105057	1.6627141902582185
0.8933618798884035	1.6626947454347194
0.894025512844199	1.662654918173672
0.8953527787557898	1.662571454872572
0.8980073105789717	1.662388812581141
0.8983170931600063	1.6623660932253215
0.8986268757410409	1.6623430736831017
0.8992464409031103	1.6622961264701785
0.900485571227249	1.66219854573527
0.9029638318755265	1.661988196111017
0.9032736144565612	1.6619604388311457
0.9035833970375959	1.6619323493415028
0.9042029621996652	1.6618751651702288
0.905442092523804	1.6617567151647747
0.9079203531720814	1.6615029864987774
0.9082301357531161	1.661469647690361
0.9085399183341507	1.6614359403564969
0.9091594834962201	1.661367410373299
0.9103986138203588	1.6612258198336176
0.9128768744686363	1.6609239442808468
0.9178333957651912	1.660240533813997
0.9181370883269139	1.6601950061001094
0.9184407808886366	1.6601490387762472
0.9190481660120818	1.6600557732077619
0.9202629362589725	1.6598638322248425
0.9226924767527537	1.659457597749053
0.9229961693144764	1.6594046586541844
0.923299861876199	1.6593512282680796
0.9239072469996443	1.6592428796320335
0.9251220172465349	1.6590201311103354
0.9275515577403162	1.6585496015769838
0.9278552503020389	1.6584883639084125
0.9281589428637615	1.6584265749277702
0.9287663279872068	1.658301326710681
0.9299810982340975	1.6580440327148802
0.9324106387278788	1.657501286092654
0.9372697197154413	1.6562947806711994
0.937599210012954	1.6562067358727823
0.9379287003104666	1.6561178608856615
0.938587680905492	1.6559375911022136
0.9399056420955427	1.6555667625011872
0.9425415644756441	1.6547821900116304
0.9428710547731567	1.6546799345678784
0.9432005450706694	1.6545767206693291
0.9438595256656948	1.6543673816983804
0.9451774868557454	1.653936801640991
0.9478134092358468	1.6530258661226396
0.9481428995333594	1.652907134147823
0.9484723898308721	1.6527872854191252
0.9491313704258975	1.6525441930909364
0.9504493316159481	1.6520441075031085
0.9530852539960496	1.6509856138440515
0.9583570987562524	1.6486108929836822
0.9586645551569021	1.6484607882738094
0.9589720115575517	1.6483093158422375
0.959586924358851	1.6480022077767749
0.9608167499614495	1.6473709043934137
0.9632764011666465	1.6460362433323816
0.9635838575672961	1.645862311432613
0.9638913139679457	1.645686739352177
0.964506226769245	1.6453305954108677
0.9657360523718435	1.6445977326527041
0.9681957035770405	1.64304475646838
0.9685031599776902	1.642841990849176
0.9688106163783399	1.6426372194103425
0.9694255291796391	1.6422215505879874
0.9706553547822376	1.6413649166045605
0.9731150059874347	1.639543572386581
0.9734224623880844	1.6393051192156636
0.973729918788734	1.6390641483112538
0.9743448315900333	1.6385744972802636
0.9755746571926318	1.637563209908572
0.9780343083978288	1.635402554051279
0.9783775220102351	1.6350853091503157
0.9787207356226415	1.6347639713576574
0.9794071628474543	1.6341086803658211
0.9807800172970798	1.6327451117027916
0.9811232309094862	1.632392616261941
0.9814664445218926	1.6320352715817192
0.9821528717467053	1.6313055865474968
0.9835257261963308	1.6297828411047026
0.9838689398087372	1.6293881852504284
0.9842121534211435	1.6289876561535055
0.9848985806459563	1.6281683559168905
0.9862714350955818	1.6264520096730863
0.9868772660121116	1.625615781056906

==> second-moment-data2.tex <==
2.040816326530612e-8	1.5862946797138147
0.00030671792055962676	1.5881334975147805
0.0006134154329559882	1.5895487074785195
0.0009201129453523496	1.5908048019344523
0.0012268104577487112	1.591958035812918
0.0015335079701450727	1.5930351246930732
0.001840205482541434	1.5940518013822316
0.002453600507334157	1.5959424875237436
0.002760298019730519	1.5968294047223524
0.00306699553212688	1.5976834965605635
0.003680390556919603	1.5993062662290818
0.004907180606505049	1.6022741136667809
0.005213878118901411	1.6029679162612793
0.0055205756312977725	1.6036449520731748
0.006133970656090495	1.6049526149175417
0.0073607607056759405	1.60740443348111
0.009814340804846833	1.611781263837537
0.010121038317243194	1.6122871538796468
0.010427735829639555	1.612784964375167
0.011041130854432278	1.6137574088615354
0.012267920904017723	1.6156162221059691
0.014721501003188616	1.6190331867080798
0.015028198515584977	1.619435275213858
0.01533489602798134	1.619832258670457
0.015948291052774063	1.6206113919734433
0.017175081102359508	1.622113436530571
0.0196286612015304	1.6249142885170522
0.01996115644971678	1.6252748070448275
0.020293651697903155	1.6256310790603492
0.020958642194275914	1.6263312271906822
0.022288623187021427	1.6276841905823818
0.024948585172512458	1.6302167890009625
0.025281080420698838	1.6305183564001196
0.025613575668885218	1.6308167802141516
0.026278566165257974	1.631404407956244
0.02760854715800349	1.6325441828582994
0.03026850914349452	1.6346919749763849
0.0306010043916809	1.634948902017146
0.03093349963986728	1.6352033894030162
0.03159849013624004	1.6357051864012773
0.03292847112898555	1.6366810139646435
0.035588433114476584	1.6385285678581303
0.040908357085458646	1.6418550756356982
0.04121881843678198	1.6420355457632592
0.04152927978810532	1.6422146155509578
0.042150202490751985	1.6425686147938698
0.043392047896045324	1.6432604631995762
0.04587573870663201	1.6445826603164837
0.05084312032780537	1.6470032055023656
0.05115358167912871	1.6471453660215607
0.051464043030452045	1.6472865138165322
0.05208496573309871	1.647565808917065
0.05332681113839205	1.6481126539533006
0.05581050194897873	1.6491613188374876
0.06077788357015209	1.6510927736685075
0.0610822549021634	1.6512044332216393
0.06138662623417471	1.6513153589898022
0.06199536889819733	1.6515350329574559
0.06321285422624258	1.6519658334016771
0.06564782488233308	1.6527944934650316
0.07051776619451407	1.6543292681036237
0.07082213752652539	1.654420103641691
0.07112650885853669	1.654510367296251
0.07173525152255932	1.65468919585741
0.07295273685060456	1.6550401739729712
0.07538770750669506	1.65571630853691
0.08025764881887605	1.6569719512492433
0.08058781788667738	1.657052685891637
0.08091798695447872	1.6571328857472096
0.08157832509008137	1.6572916970041822
0.0828990013612867	1.6576030749114459
0.08554035390369732	1.6582016952694376
0.09082305898851858	1.6593086835265634
0.09115322805631991	1.659374107278295
0.09148339712412124	1.659439106887139
0.0921437352597239	1.659567845510308
0.09346441153092921	1.6598203617841256
0.09610576407333984	1.6603061809690987
0.10138846915816112	1.6612057011432952
0.10169660432909941	1.661255364679843
0.10200473950003769	1.6613047312965725
0.10262100984191426	1.6614025811338031
0.1038535505256674	1.661594798004465
0.10631863189317368	1.6619656957120261
0.11124879462818625	1.662656341654146
0.11155692979912454	1.662697354962702
0.11186506497006282	1.6627381241749026
0.11248133531193939	1.6628189361591217
0.11371387599569253	1.6629776947482042
0.11617895736319882	1.6632840652884675
0.12110912009821138	1.6638546151411222
0.12144305300493968	1.6638913243524756
0.121776985911668	1.6639277966584605
0.12244485172512459	1.664000036558539
0.12378058335203782	1.6641417389587356
0.12645204660586423	1.6644143572633874
0.1317949731135171	1.6649189044212476
0.1321289060202454	1.6649487297245529
0.1324628389269737	1.6649783614795286
0.13313070474043032	1.6650370491801052
0.1344664363673435	1.665152154755101
0.13713789962116996	1.6653735474973166
0.1424808261288228	1.665783049374259
0.14280866901623906	1.6658068050446768
0.14313651190365534	1.6658304080194453
0.14379219767848792	1.6658771596188522
0.14510356922815304	1.6659688712624054
0.14772631232748326	1.6661453305186484
0.15297179852614373	1.6664719406706217
0.15329964141356	1.6664912477489833
0.15362748430097628	1.66651042948551
0.15428317007580886	1.6665484200306464
0.15559454162547398	1.6666229308473586
0.1582172847248042	1.666766239301325
0.16346277092346467	1.6670312918780092
0.16376857991401791	1.6670459026437978
0.16407438890457116	1.667060424132972
0.1646860068856776	1.6670892013874643
0.16590924284789055	1.667145707595251
0.16835571477231645	1.6672546413891687
0.17324865862116823	1.667457077768712
0.17355446761172147	1.6674690805772852
0.1738602766022747	1.6674810097420258
0.17447189458338117	1.6675046489381713
0.1756951305455941	1.6675510632635628
0.17814160247001998	1.6676405336035984
0.18303454631887175	1.6678067973463064
0.18336615304521503	1.6678174854468109
0.18369775977155828	1.6678281027372173
0.18436097322424477	1.667849126857087
0.18568740012961776	1.6678903469011424
0.1883402539403638	1.6679695813717588
0.19364596156185587	1.668116054082311
0.19397756828819912	1.6681247090601428
0.19430917501454237	1.6681333078514717
0.1949723884672289	1.6681503385572292
0.1962988153726019	1.6681837441268017
0.19895166918334792	1.668248023566672
0.20425737680483996	1.6683671634496497
0.20456694963432018	1.6683737522387245
0.2048765224638004	1.6683803029602062
0.2054956681227608	1.6683932913779964
0.20673395944068162	1.6684188242852345
0.20921054207652331	1.6684681787207696
0.21416370734820667	1.6685605405820518
0.21447328017768688	1.6685660513178402
0.2147828530071671	1.6685715328186321
0.2154019986661275	1.6685824091429886
0.21664028998404833	1.6686038222172563
0.21911687261989002	1.6686453462614994
0.22407003789157337	1.668723621803114
0.22437352070174155	1.6687282272565898
0.22467700351190975	1.6687328120333278
0.22528396913224613	1.6687419204054426
0.22649790037291886	1.6687598983192875
0.22892576285426436	1.6687949452923543
0.23378148781695532	1.6688617647858932
0.24349293774233727	1.668985031188786
0.26456689268366235	1.6692282582447684
0.2842306782257526	1.6694597472093435
0.2845637226106378	1.6694639060657732
0.2848967669955229	1.6694680757744458
0.2855628557652933	1.6694764482883568
0.286895033304834	1.6694933294527519
0.2895593883839155	1.6695276659072296
0.2948880985420783	1.6695988653617622
0.305545518858404	1.6697531106274652
0.30587247322397715	1.6697581227878444
0.30619942758955027	1.6697631528230505
0.30685333632069656	1.6697732669197491
0.3081611537829892	1.6697937140105212
0.3107767887075744	1.6698355058175531
0.3160080585567449	1.6699228515051319
0.32647059825508584	1.6701138917528486
0.32677551872379595	1.6701198079229984
0.32708043919250607	1.6701257446392324
0.3276902801299263	1.6701376799686167
0.32890996200476674	1.6701618000135485
0.33134932575444764	1.6702110518561228
0.3362280532538094	1.6703137133962138
0.34598550825253294	1.6705365113189363
0.3463162264570331	1.6705444875125761
0.3466469446615332	1.670552492271996
0.3473083810705334	1.6705685877540255
0.34863125388853394	1.670601124418162
0.35127699952453495	1.6706675951231076
0.356568490796537	1.6708062394815062
0.3671514733405411	1.6711071988295627
0.3674601576481782	1.671116465158569
0.3677688419558153	1.6711257596788731
0.36838621057108945	1.671144433463739
0.3696209478016378	1.6711821211946354
0.3720904222627345	1.6712588666489179
0.3770293711849278	1.6714179103409963
0.3869072690293145	1.6717587609158688
0.3872417510727416	1.6717708446693773
0.38757623311616873	1.6717829643923394
0.3882451972030229	1.6718073119181989
0.38958312537673134	1.671856440480867
0.39225898172414814	1.671956441034526
0.3976106944189818	1.6721634886454833
0.408314119808649	1.6726063168014869
0.429331209352014	1.6735910099248383
0.44893812949614426	1.6746522307348597
0.47019610473083556	1.6759632275713927
0.4900439105662921	1.677340816239213
0.5095019551657791	1.6788366463802702
0.5306110548558273	1.6806220746115677
0.5503099851466406	1.682439547461282
0.5716599705280151	1.6845711138334611
0.5926201946734201	1.6868224067677071
0.6121702494195903	1.6890576527694585
0.6333713592563216	1.6916203655519484
0.6531622996938181	1.6941321824644122
0.6725634788953451	1.6966940335429823
0.6936157131874332	1.6995677384757848
0.7132577780802865	1.7023164648952873
0.7345508980637009	1.705340831037797
0.7544338486478805	1.7081729764796265
0.7739270379960906	1.7109170608445994
0.7950712824348619	1.7137993899174777
0.8148053574743983	1.7163306576522854
0.8151395001326811	1.716371706774733
0.8154736427909639	1.716412686235761
0.8161419281075294	1.7164944341887618
0.8174784987406605	1.7166570721837244
0.8201516400069226	1.7169788020889392
0.8254979225394471	1.717607126009594
0.8361904876044959	1.7187949913983926
0.8365185402434666	1.718829821790872
0.8368465928824373	1.71886454887456
0.8375026981603789	1.71893369048277
0.838814908716262	1.7190707048307619
0.8414393298280279	1.7193395058962602
0.84668817205156	1.719854928349625
0.8470162246905307	1.7198861080998487
0.8473442773295015	1.7199171615954707
0.8480003826074429	1.719978886675372
0.849312593163326	1.7201007869022058
0.8519370142750919	1.7203382054078595
0.857185856498624	1.720785991220461
0.8574918752407317	1.7208109271308887
0.8577978939828395	1.7208357292469807
0.8584099314670548	1.7208849290132344
0.8596340064354857	1.7209816888553138
0.8620821563723473	1.7211684713798634
0.862388175114455	1.721191171719153
0.8626941938565627	1.7212137254072843
0.8633062313407781	1.7212583894509283
0.8645303063092089	1.7213459202759793
0.8669784562460706	1.7215135971526476
0.8672844749881783	1.721533847020166
0.8675904937302861	1.7215539361272068
0.8682025312145014	1.7215936283461226
0.8694266061829323	1.7216710424927215
0.8718747561197939	1.7218177742984155
0.8721807748619016	1.7218353375517772
0.8724867936040093	1.7218527245180624
0.8730988310882247	1.7218869654962394
0.8743229060566555	1.7219532866254588
0.8767710559935172	1.7220770479945722
0.8771028724714149	1.722092887764229
0.8774346889493128	1.7221085000117524
0.8780983219051082	1.7221390361660203
0.879425587816699	1.7221973141254616
0.8797574042945967	1.7222112928007747
0.8800892207724944	1.7222250321399062
0.8807528537282899	1.7222517867038583
0.8820801196398809	1.7223023560254733
0.8824119361177786	1.7223143767362112
0.8827437525956763	1.7223261456135324
0.8834073855514717	1.7223489214051677
0.8847346514630626	1.7223913792407408
0.8850664679409603	1.7224013394681492
0.8853982844188582	1.7224110346284753
0.8860619173746536	1.722429622899975
0.8873891832862444	1.7224635426020887
0.8877209997641421	1.72247133373458
0.8880528162420398	1.7224788457712892
0.8887164491978353	1.7224930252932578
0.889048265675733	1.722499689112433
0.8893800821536308	1.7225060665033902
0.8900437151094263	1.722517954515819
0.890375531587324	1.7225234613594576
0.8907073480652217	1.722528674218932
0.8910391645431194	1.7225335911692694
0.8913709810210171	1.7225382102708091
0.8917027974989148	1.7225425295690564
0.8920346139768125	1.722546547094527
0.8923664304547103	1.7225502608625953
0.892698246932608	1.722553668873343
0.8930300634105057	1.7225567691113937
0.8933618798884035	1.7225595595457621
0.8936936963663012	1.7225620381296802
0.894025512844199	1.7225642028004498
0.8943573293220967	1.7225660514792653
0.8946891457999944	1.7225675820710482
0.8950209622778921	1.7225687924642785
0.8953527787557898	1.7225696805308197
0.8956845952336875	1.7225702441257462
0.8960164117115852	1.7225704810871645
0.896348228189483	1.7225703892360338
0.8966800446673807	1.7225699663759866
0.8970118611452784	1.7225692102931391
0.8973436776231762	1.7225681187559088
0.897675494101074	1.722566689514824
0.8980073105789717	1.7225649203023288
0.8983170931600063	1.722562959697298
0.8986268757410409	1.7225606989058666
0.8989366583220757	1.7225581360392939
0.8992464409031103	1.72255526919452
0.899556223484145	1.7225520964540166
0.8998660060651797	1.7225486158856431
0.900485571227249	1.7225407234627652
0.9007953538082838	1.722536307669561
0.9011051363893184	1.7225315761707756
0.9017247015513878	1.7225211580109867
0.9020344841324225	1.7225154672882288
0.9023442667134571	1.722509452736062
0.9029638318755265	1.7224964438448196
0.9032736144565612	1.7224894453157367
0.9035833970375959	1.7224821145768823
0.9042029621996652	1.7224664479071854
0.9045127447807	1.722458107652588
0.9048225273617346	1.7224494265403503
0.905442092523804	1.7224310329048846
0.9057518751048387	1.722421315918365
0.9060616576858733	1.722411249147238
0.9066812228479427	1.7223900571256834
0.9079203531720814	1.7223433742451948
0.9082301357531161	1.7223307941875667
0.9085399183341507	1.7223178456044912
0.9091594834962201	1.72229083312287
0.9103986138203588	1.7222322775863423
0.9107083964013936	1.7222166801511092
0.9110181789824282	1.7222006941771268
0.9116377441444976	1.7221675462032824
0.9128768744686363	1.7220964720398793
0.913186657049671	1.7220776923326666
0.9134964396307057	1.722058502681768
0.914116004792775	1.7220188824049796
0.9153551351169138	1.7219345985788101
0.9178333957651912	1.7217452015856438
0.9181370883269139	1.721720024526025
0.9184407808886366	1.7216944078564316
0.9190481660120818	1.7216418435964835
0.9202629362589725	1.7215313052306391
0.9205666288206951	1.7215025253121705
0.9208703213824178	1.7214732808829536
0.921477706505863	1.7214133854988218
0.9226924767527537	1.7212878759889993
0.9229961693144764	1.721255287548399
0.923299861876199	1.7212222078165629
0.9239072469996443	1.7211545604890541
0.9251220172465349	1.7210132145844308
0.9275515577403162	1.7207054902852288
0.9278552503020389	1.7206646032709259
0.9281589428637615	1.7206231649445525
0.9287663279872068	1.720538618036001
0.9299810982340975	1.7203627266572747
0.9324106387278788	1.7199827852691978
0.9327143312896015	1.719932565139224
0.9330180238513242	1.7198817233881822
0.9336254089747694	1.7197781558097702
0.9348401792216601	1.7195633469751506
0.9372697197154413	1.7191018903160424
0.937599210012954	1.7190359248964928
0.9379287003104666	1.7189691292882396
0.938587680905492	1.718833018262527
0.9399056420955427	1.7185505071769713
0.9425415644756441	1.717942569718356
0.9428710547731567	1.7178623936534716
0.9432005450706694	1.7177812591337904
0.9438595256656948	1.7176160789205768
0.9451774868557454	1.7172738163786578
0.9478134092358468	1.7165395158912478
0.9481428995333594	1.716442863295299
0.9484723898308721	1.7163450939454685
0.9491313704258975	1.7161461603750157
0.9504493316159481	1.715734392302658
0.9530852539960496	1.7148525336745424
0.9534147442935623	1.7147365832399193
0.9537442345910749	1.7146193169787582
0.9544032151861004	1.7143807802387725
0.9557211763761511	1.7138872798347409
0.9583570987562524	1.7128310828760558
0.9586645551569021	1.7127015810379715
0.9589720115575517	1.7125707114781883
0.959586924358851	1.7123048091563027
0.9608167499614495	1.7117559172600958
0.9632764011666465	1.7105860791733722
0.9635838575672961	1.7104327501453924
0.9638913139679457	1.7102777809367449
0.964506226769245	1.7099628427390128
0.9657360523718435	1.7093123914680035
0.9681957035770405	1.7079242382579882
0.9685031599776902	1.7077420755105726
0.9688106163783399	1.7075579069435276
0.9694255291796391	1.7071834438647495
0.9706553547822376	1.7064092213684772
0.9731150059874347	1.7047527001248062
0.9734224623880844	1.7045348498256774
0.973729918788734	1.704314481793056
0.9743448315900333	1.703866036505643
0.9755746571926318	1.7029371606211057
0.9780343083978288	1.7009413277381216
0.9783775220102351	1.7006470818251045
0.9787207356226415	1.700348743020392
0.9794071628474543	1.699739450004448
0.9807800172970798	1.698467877293203
0.9811232309094862	1.6981383808402983
0.9814664445218926	1.697804035148023
0.9821528717467053	1.6971203480896926
0.9835257261963308	1.695689598598683
0.9838689398087372	1.695317941732355
0.9842121534211435	1.6949404116233782
0.9848985806459563	1.6941671093626556
0.9862714350955818	1.6925427590706357
0.9890171439948328	1.68893684806465
0.9893603576072392	1.6884477039850183
0.9897035712196455	1.6879490005250848
0.9903899984444582	1.686921435570151
0.9917628528940837	1.6847337250345649
0.99210606650649	1.684156284176358
0.9924492801188964	1.6835654766095038
0.9931357073437093	1.682341004913667
0.9945085617933347	1.679697111303799
0.9948517754057411	1.6789894590517573
0.9951949890181475	1.6782605189043605
0.9958814162429602	1.6767319950767439
0.9962246298553665	1.6759283262985756
0.9965678434677729	1.675095049400798
0.9972542706925858	1.6733264599010134
0.9975974843049922	1.6723825256285827
0.9979406979173985	1.6713910562584506
0.9982839115298048	1.6703437874568392
0.9986271251422112	1.6692290887296166
0.9989703387546176	1.6680293550954037
0.999313552367024	1.6667146918839004
0.9996567659794304	1.6652221470818644
0.9999999795918367	1.6632557177086666
